Document Spanners for Extracting Incomplete Information: Expressiveness and Complexity

Rule-based information extraction has lately received a fair amount of attention from the database community, with several languages appearing in the last few years. Although information extraction systems are intended to deal with semistructured data, all language proposals introduced so far are designed to output relations, thus making them incapable of handling incomplete information. To remedy the situation, we propose to extend information extraction languages with the ability to use mappings, thus allowing us to work with documents which have missing or optional parts. Using this approach, we simplify the semantics of regex formulas and extraction rules, two previously defined methods for extracting information, extend them with the ability to handle incomplete data, and study how they compare in terms of expressive power. We also study computational properties of these languages, focusing on the query enumeration problem, as well as satisfiability and containment.

==> Evaluation.tex <==
%!TEX root = main.tex

%\section{Evaluation of IE languages}\label{sec:evaluation}
\section{Evaluation of languages extracting incomplete data}\label{sec:evaluation}

In this section, we study the computational complexity of evaluating an extraction expression $\gamma$ over a document $d$, namely, the complexity of enumerating all mappings $\mu \in \semd{\gamma}$.
Given that we are dealing with an enumeration problem, our objective is to obtain an \emph{incremental polynomial time} algorithm~\cite{johnson1988generating}, i.e., an algorithm that enumerates all the mappings in $\semd{\gamma}$ by taking  time polynomial in the size of $\gamma$ and $d$ between outputting two consecutive results.
For this analysis, we model our problem as a decision problem and relate it to the enumeration problem.
Formally, let $\bot$ be a new symbol. 
An \emph{extended mapping} $\mu$ over $d$ is a partial function from $\VV$ to $\sub(d) \cup \{\bot\}$.
Intuitively, in our decision problem $\mu(x) = \bot$ will represent that the variable $x$ will not be mapped to any span.
Furthermore, we usually treat $\mu$ as a normal mapping by assuming that $x$ is not in $\dom(\mu)$ for all variables $x$ that are mapped to $\bot$.
Given two extended mappings $\mu$ and $\mu'$, we say that $\mu \subseteq \mu'$ if, and only if, $\mu(x) = \mu'(x)$ for every $x \in \dom(\mu)$. 
%We denote by $\mu_{\downarrow}$ the maximum mapping who satisfies that $\mu_{\downarrow} \subseteq \mu$ and $x \notin \dom(\mu_\downarrow)$ whenever $\mu(x) = \bot$.
Then for any language $\LL$ for information extraction we define the main decision problem for evaluating expressions from $\LL$:
\begin{center}
	\framebox{
		\begin{tabular}{rl}
			\textbf{Problem:} & $\EVAL[\LL]$\\
			\textbf{Input:} &  An expression $\gamma \in \LL$, a document $d$,  
			 and an extended mapping $\mu$.  \\
			\textbf{Question:} & Does there exist $\mu'$ such that 
			  $\mu \subseteq \mu'$ and  $\mu' \in \semd{\gamma}$?
		\end{tabular}
	}
\end{center}
In other words, in $\EVAL[\LL]$ we want to check whether $\mu$ can be extended to a mapping $\mu'$ that satisfies $\gamma$ in $d$.
Note that in our analysis we will consider the combined complexity of $\EVAL[\LL]$.
%We believe that, although the data complexity of the problem (i.e. the expression $\gamma$ is not part of the input) could derive an interesting insight in the evaluation of extraction expressions, it will not model correctly the complexity in this case.
%
%
We claim that $\EVAL[\LL]$ correctly models the problem of enumerating all mappings in $\semd{\gamma}$. 
Indeed, if we can find a polynomial time algorithm for deciding $\EVAL[\LL]$, then we can define an incremental polynomial time algorithm for computing $\semd{\gamma}$. % as follows. %presented in Algorithm \ref{alg:enum}.
 More precisely, we define a recursive procedure $\ENUM(\gamma, d, \mu, V)$ that, when started with $\mu = \emptyset$ and $V=\Var(\gamma)$ enumerates all $\mu \in \semd{\gamma}$. The procedure simply picks a variable $x \in V$ and iterates over all $s \in \sub(d)$ (or the symbol $\bot$ signalling that $x$ is not assigned) and checks if $\EVAL[\LL](\gamma, d, \mu[x \rightarrow s])$ is true where $\mu[x \rightarrow s]$ is an extended mapping where $x$ is assigned to $s$. If this is the case we then recursively call $\ENUM(\gamma, d, \mu[x \rightarrow s], V\backslash \{x\})$. Once $V$ becomes empty (meaning all the variables have been assigned a span or $\bot$) we simply output the mapping $\mu$. It is straightforward to check that this procedure efficiently enumerates all spans in $\semd{\gamma}$, if we can decide $\EVAL[\LL]$ efficiently.
%
%
%\begin{algorithm}
%  \caption{Enumerate all spans in \(\semd{\gamma}\), where \(\mu\) is the
%    current mapping and \(V\) is the set of available variables.}
%  \label{alg:enum}
%  \begin{algorithmic}[1]
%    \Procedure{Enumerate}{$\gamma, d, \mu, V$}
%      \If{\(V = \emptyset\)}
%        \State{\textbf{output} \(\mu\) and \Return}
%      \EndIf
%      \State{Let \(x\) be some element from \(V\)}
%      \For{\(s \in \sub(d) \cup \{\bot\}\)}
%        \If{\(\EVAL[\LL](\gamma, d, \mu[x \to s])\)}
%          \State{
%            \Call{Enumerate}{$\gamma, d, \mu[x \to s], V\,\setminus\,\{x\}$}}
%        \EndIf
%      \EndFor
%    \EndProcedure
%  \end{algorithmic}
%\end{algorithm}
%
%The procedure starts with the empty mapping $\mu = \emptyset$ and the set $V$ of variables yet to be assigned equal to $\Var(\gamma)$. 
%For a variable $x \notin \dom(\mu)$ we iterate over all $s \in \sub(d)$ (or the symbol $\bot$ signalling that $x$ is not assigned) and check if $\EVAL[\LL](\gamma, d, \mu[x \rightarrow s])$ is true where $\mu[x \rightarrow s]$ is an extended mapping where $x$ is assigned to $s$ (lines 5 through 7).
%If the answer is positive, then in line 8 we recursively continue with the mapping $\mu[x \rightarrow s]$ (i.e. we know that the set of answers is non-empty).
%%After iterating over all spans that can be assigned to $x$, the last case is to consider all mappings where $x$ is not assigned (i.e. $x$ is assigned to $\bot$). Thus, we check whether $\EVAL[\LL](\gamma, d, \mu[x \rightarrow \bot])$ holds and continue recursively with $\mu[x \rightarrow \bot]$ if the answer is positive. 
%Finally, we print the mapping $\mu$ when all variables in $\Var(\gamma)$ are assigned a span or the symbol $\bot$ (i.e. $V=\emptyset$ in line 2). 
%%(i.e. $\dom(\mu) = \Var(\gamma)$). 
%It is straightforward to check that this procedure efficiently enumerates all spans in $\semd{\gamma}$, if we can decide $\EVAL[\LL]$ efficiently.
\begin{proposition}\label{prop:evaluation}
	If $\EVAL[\LL]$ is in $\PTIME$, then enumerating all spans in $\semd{\gamma}$ can be done in incremental polynomial time.
\end{proposition}
Two decision problems associated with $\EVAL[\LL]$, that have a long standing history in data management~\cite{AHV95}, are \emph{model checking} and the \emph{non-emptiness problem}.
Formally, the model checking problem (non-emptiness problem), denoted by $\mdcheck[\LL]$ ($\nemp[\LL]$ resp.), asks whether $\mu \in \semd{\gamma}$ ($\semd{\gamma} \neq \emptyset$ resp.) for any $\gamma \in \LL$, document~$d$ and mapping $\mu$.
One can easily see that  both problems are actually restricted instances of $\EVAL[\LL]$, namely:
$$
\renewcommand{\arraystretch}{1.1}
\begin{array}{rcl}
\mdcheck[\LL](\gamma, d, \mu) & = & \EVAL[\LL](\gamma, d, \mu_\bot) \\
\nemp[\LL](\gamma, d) & = & \EVAL[\LL](\gamma, d, \emptyset) 
\end{array}
$$
where $\mu_\bot$ is the extended mapping such that, for all $x \in \Var(\gamma)$, it holds that $\mu_\bot(x) = \mu(x)$ if $x \in \dom(\mu)$ and $\bot$ otherwise.
This implies that if we find an efficient algorithm for $\EVAL[\LL]$ then the same holds for $\mdcheck[\LL]$ and $\nemp[\LL]$.
In contrast, if we show that $\mdcheck[\LL]$ or $\nemp[\LL]$ are $\NP$-hard, then we will have that $\EVAL[\LL]$ is $\NP$-hard and, consequently, the enumeration of $\semd{\gamma}$ will be inefficient.
We use these relations to simplify results that follow.
%
%
%In order to understand the complexity of this problem with respect to the classical computational complexity theory, we must model our problem as a decision problem. 
%The usual way of modeling this as a decision problem is to consider the problem of checking whether a span $s$ is in the output set $\semd{\gamma}$  given an extraction expression $\gamma$ and a document $d$. 
%Unfortunately, this decision version of the evaluation problem does not model exactly the real complexity behind the problem in the sense that an efficient algorithm (i.e. $\PTIME$) for this will not give necessarily an efficient algorithm for evaluating extraction expressions (i.e. computing all spans in $\semd{\gamma}$).
%For this reason, we consider the following decision version of the evaluation problem. For any language $\LL$ for span extraction we define:
%\begin{center}
%\framebox{
%	\begin{tabular}{rl}
%		\textbf{Problem:} & $\nemp(\LL)$\\
%		\textbf{Input:} & A document $d$ and an expression $\gamma \in \LL$.\\
%		\textbf{Question:} & Is $\semd{\gamma}$ not empty?
%	\end{tabular}
%}
%\end{center}
%We claim that decision problem $\nemp(\LL)$ correctly models the problem of enumerating all mappings in $\semd{\gamma}$. 
%Indeed, if $\nemp(\LL)$ is hard, then $\semd{\gamma}$ will also be hard (i.e. if I can compute $\semd{\gamma}$ efficiently, then I will decide $\nemp(\LL)$ efficiently too).
%In the other direction, if I can find an efficient algorithm for deciding $\nemp(\LL)$, one can have an efficient algorithm for computing $\semd{\gamma}$ as follows: for any variable $x$ in $\gamma$, iterate over all spans $s$ in $d$ and check whether $\semd{\gamma}$ is non empty when $x$ is replaced by $s$. 
%If the answer is positive, then continue with the next variable by finding all mappings where $x$ is assigned to $s$ (we know that this set is non-empty). Otherwise, consider the next span for $x$ and iterate. 
%One can easily check that this gives a \emph{polynomial total time} algorithm~\cite{johnson1988generating} for enumerating $\gamma$ in the size of $|\gamma|$, $|d|$ and $|\semd{\gamma}|$ (note that the size of the output is also included in the analysis).
%In the last claim, we are supposing that an algorithm for $\nemp(\LL)$ can be extended for formulas $\gamma[x \rightarrow s]$ where a variable $x$ is restricted to a span $s$. As we will see, this is always possible in the algorithm presented in this paper. 


Now that we identified the appropriate decision problem, we start by understanding the complexity of $\EVAL(\LL)$ in the most general case.
First of all, one can see that checking $\EVAL(\LL)$ is in $\NP$ for all languages and computational models considered in this paper.
Indeed, given a mapping $\mu'$ such that $\mu \subseteq \mu'$ one can check in $\PTIME$ if $\mu' \in \semd{\gamma}$ by using finite automata evaluation techniques~\cite{HopcroftU79}.
As the following result shows, this is the best that one can do if $\RGX$ or variable-set automata contain the language of $\SRGX$.
\begin{theorem}\label{theo:hardness-general}
$\nemp[\SRGX]$ is $\NP$-comp.
\end{theorem}
We would like to remark that this result was proved in \cite{AMRV16} and here we just rephrased it in light of the new framework presented in this paper.

The previous result implies that the evaluation problem for $\RGX$ and variable-set automata is $\NP$-complete. However, it does not say anything about the model checking problem.
By adapting the proof of the previous result it can be shown that, unfortunately, the model checking problem is also hard for $\RGX$ and variable automata.
% Interestingly, the model checking problem becomes tractable for $\RGX$ expressions but, unfortunately, it is hard for variable-set automata.
\begin{theorem}\label{theo:model-check}
  $\mdcheck[\SRGX]$ is $\NP$-complete.
\end{theorem}
% The previous result justifies the complexity analysis divided into different decision problems: although the model checking problem of $\RGX$ is tractable, this is not enough for getting $\PTIME$-algorithms for evaluating~them.
% That is, if our analysis only considered the model checking problem, we could wrongly assume that computing $\semd{\gamma}$ can be done efficiently for a \RGX\ $\gamma$.
%That is, if our analysis could be restricted to the model checking problem, we could wrongly state that evaluation of $\RGX$ is tractable when it is not.

With the previous negative results, we examine several syntactical restrictions of $\RGX$ and variable-set automata that make the evaluation problem tractable.
Note that the previous negative results are considering a more general setting than the one presented in~\cite{FKRV15}, where $\RGX$ and variable-set automata are restricted to be \emph{functional} which forces them to only generate relations of spans. 
Interestingly, the functional restriction decreases the complexity of the evaluation problem for $\RGX$ as the following result shows.
\begin{proposition}\label{theo:ptime-functional-RGX}
	$\EVAL[\fRGX]$ is in $\PTIME$.
\end{proposition}
This result proves that the functional restriction for $\RGX$ introduced in~\cite{FKRV15} is crucial for getting tractability. 
The question that now remains is what the necessary restrictions are that make the evaluation of $\RGX$ tractable when outputting mappings and how to extend these restrictions to other classes like variable-set automata.
One possible approach is to consider variable-set automata that produce only relations. 
Formally, we say that a variable-set automaton $\cA$ is \emph{relational} if for all documents $d$, the set $\semd{\cA}$ forms a relation. 
As the next result shows, this semantic restriction is not enough to force tractability on $\EVAL[\VA]$.
\begin{proposition}\label{theo:hardness-relational-VA}
	$\mdcheck$ and $\nemp$ of relational VA automata are $\NP$-complete.
\end{proposition}
By taking a close look at the proof of the previous result, one can note that a necessary property for getting intractability is that, during a run, the automaton can see the same variable on potential transitions many times but not use it if it has closed the same variable in the past.
Intuitively, this cannot happen in functional $\RGX$ formulas where for every subformula of the form $\varphi_1 \cdot \varphi_2$ it holds that $\Var(\varphi_1) \cap \Var(\varphi_2) =
\emptyset$.
Actually, we claim that this is the restriction that implies tractability for evaluating $\RGX$ formulas. 
Formally, we say that a $\RGX$ formula $\gamma$ is \emph{sequential} if for every subformula of the form $\varphi_1 \cdot \varphi_2$ or $\varphi^*$ it holds that $\Var(\varphi_1) \cap \Var(\varphi_2) =
\emptyset$ and $\Var(\varphi) = \emptyset$, respectively.
We can also extend these ideas of sequentiality from $\RGX$ formulas to variable-set automata as follows.
A path $\pi$ of a variable-set automaton $\cA = (Q, q_0, q_f, \delta)$ is a finite sequence of transitions 
$\pi: (q_1, s_2, q_2), (q_2, s_3, q_3) \ldots, (q_{m-1}, s_m, q_m)$ such that $(q_i, s_{i+1}, q_{i+1}) \in
\delta$ for all $i \in [1, m - 1]$.
We say that a path $\pi$ of $\cA$ is sequential if for every variable \(x \in
\VV\) it holds that: (1) there is at most one \(i \in [1, m]\) such that \(s_i =
\Open{x}\); (2) there is at most one \(j \in [1, m]\) such that \(s_j = \Close{x}\); and (3) if such a \(j\)
exists, then \(i\) exists and \(i < j\).
We say that variable-set automaton $\cA$ is sequential if every path in $\cA$ is sequential.
Finally, we denote the class of sequential RGX and sequential variable-set automata by $\seqRGX$ and $\seqVA$, respectively.

The first natural question about sequentiality is whether this property can be checked efficiently. As the next proposition shows, this is indeed the case.
%sequentiality can be checked in $\NLOGSPACE$.
\begin{proposition}\label{theo:ptime-sequential-check}
	Deciding if an VA automaton is sequential can be done in $\NLOGSPACE$.
\end{proposition}

Sequentiality is a mild  restriction over extraction expressions since it still allows many $\RGX$ formulas that are useful in practice.
For example, all extraction expressions discussed in Section~\ref{sec-unifying} are sequential.
Furthermore, as we now show, no expressive power is lost when restricting to sequential \RGX\ or automata. %That is, we can prove the following.
%Furthermore, if we restrict to the fragment of sequential RGX and sequential variable-set automata, we can prove that we will not loose expressive power for extracting information.
\begin{proposition}\label{prop:rgx-equiv-rgx-seq}
For every \RGX\ (\VA\ automaton), there exists a sequential \RGX\ (sequential \VA, respectively) that defines the same extraction function.
\end{proposition}
We believe that sequentiality is a natural syntactical restriction of how to use variables in extraction expressions. Namely, one should not reuse variables by concatenation since this can easily make the formula unsatisfiable.
Furthermore, the more important advantage for users is that $\RGX$ and VA automata that are sequential can be evaluated efficiently. 
\begin{theorem}\label{theo:ptime-sequential-sVA}
	$\EVAL[\seqRGX]$ and $\EVAL[\seqVA]$ is in $\PTIME$.
\end{theorem}
It is important to recall that this result implies, by Proposition~\ref{prop:evaluation}, that the evaluation of sequential $\RGX$ formulas can be done in incremental polynomial time. 
Moreover, $\mdcheck$ and $\nemp$ of this class can also be decided in $\PTIME$.
This provides us with a good upper-bound for evaluating formulas and shows that it might be possible to find an efficient algorithm that works in practice. With this, we refer to a  \emph{constant delay algorithm}~\cite{johnson1988generating} like the one presented in~\cite{AMRV16} for the so-called navigational formulas -- a class strictly subsumed by sequential $\RGX$.
Thus, sequential $\RGX$ seem like a good direction for extending the constant delay algorithm for navigational formulas given in \cite{AMRV16}.
%
%navigational formulas are a good starting point for the design of constant delay algorithms and sequential $\RGX$ are a good direction for extending them.

Now that we have captured an efficient fragment of \(\RGX\), we will analyze what happens with the complexity of the evaluation problem for extraction rules. First, we show that evaluating rules is in general a hard problem. In fact, non-emptiness is already $\NP$-hard, even when restricted to functional \(\RGX\) and dag-like rules. %, evaluating rules is hard.
\begin{theorem}\label{theo:daglike-npcomplete}
  \(\nemp\) of functional dag-like rules is \(\NP\)-complete.
\end{theorem}
The difficulty in this case arises from the fact that dag-like rules allow referencing the same variable from different extraction expressions. % within the rule. %This makes the evaluation of each extraction expression highly dependent on the other extraction expressions, which makes the problem hard to solve in general.
%
%Therefore, a reasonable restriction in this case is to prohibit variables from being used in multiple extraction expression of the same rule. In other words, we will restrict ourselves to sequential tree-like rules. 
A natural way to circumvent this is to use tree-like rules. 
Indeed, the fact that, in a tree-like rule, different branches are independent, causes the evaluation problem to become tractable.
In fact, the functionality constraint is not really needed here, as the result holds even for sequential rules.
\begin{theorem}\label{theo:treelike-ptime}
  \(\EVAL\) of sequential tree-like rules is in \(\PTIME\).
\end{theorem}

This implies that we should focus on sequential tree-like rules if we wish to have efficient algorithms for rules. Luckily, these do not come at a high price in terms of expressiveness, since Theorem~\ref{thm:simple_to_dag}, Proposition~\ref{prop:nonfunc}, and Theorem~\ref{thm:dag_to_tree} imply that every satisfiable simple rule is equivalent to a union of sequential tree-like rules.

The previous results show how far we can go when syntactically restricting the class of $\RGX$ formulas, variable-set automata, or extraction rules in order to get tractability.
The next step is to parametrize the size of the query not only in terms of the length, but also in terms of meaningful parameters that are usually small in practice. 
In this direction, a natural parameter is the number of variables of a formula or automata since one would expect that this number will not be huge. 
Indeed, if we restrict the number of variables of a $\RGX$ formula or VA automata we can show that the problem is fixed parameter tractable.
\begin{theorem}\label{theo:RGX-FPT}
  $\EVAL[\RGX]$ and $\EVAL[\VA]$ parametrized by the number of variables is $\FPT$.
\end{theorem}
%Similarly, this result can be extended to unrestricted simple extraction rules.
%\begin{theorem}\label{theo:rules-FPT}
%  \(\EVAL\) of extraction rules parame-trized by the number of the number of variables is \(\FPT\).
%\end{theorem}
%The two results show that we can  evaluate all the expressions considered in this paper efficiently when assuming the number of variables to be small.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> Expressiveness-Annotation-Programs.tex <==
% Comparison of Annotation Programs vs Variable Automata.

\section{Expressiveness of Annotation Programs}

In this section, we will analyze and compare the expressiveness of
\emph{annotation programs} with that of the \emph{variable automata} defined
in~\cite{FKRV15}. For this, we distinguish a special kind of program,
\emph{non-recursive annotation programs}, that use no recursion in the
usual datalog sense.

\begin{proposition}
  For every vset-automaton there is an equivalent \emph{tree-like non-recursive
  annotation programs}.
\end{proposition}

\begin{proof}
  From~\cite{FKRV15}, we already know that $\VAStkUPJ \equiv \VASet$, and from
  Proposition~\ref{lemma:utlstar-rgx}, we know that $\RGX$ is equivalent to
  \emph{tree-like rule sets}. Therefore, it suffices to show that we may
  simulate the $\cup, \pi, \Join$ algebraic operators using non-recursive
  tree-like rules.

  To simulate \emph{union} ($\cup$) we may use \emph{rule sets}. To simulate
  \emph{projection} ($\pi$) we use may use rules of the form $A(x_1,\ldots,x_n)
  \rightarrow A_{\pi}(y_1,\ldots,y_m)$ where $\{y_1,\ldots,y_m\} \subseteq
  \{x_1,\ldots,x_n\}$. Finally, for \emph{joins} ($\Join$), we may use rules of
  the form $A(x_1,\ldots,x_n) \wedge B(y_1,\ldots,y_m) \rightarrow
  C(z_1,\ldots,z_l)$ where $\{z_1,\ldots,z_l\} = \{x_1,\ldots,x_n\} \cap
  \{y_1,\ldots,y_m\}$.
\end{proof}

Open problem:
\begin{proposition}
  \emph{Non-recursive annotation programs} and vset-automata are equivalent.
\end{proposition}


==> Expressiveness-Span-Regular-Expressions.tex <==
% Comparison of Span Regular Expressions vs Regex Formulas.

\section{Expressiveness of span regular expressions and rules}

% SRE* = RGX*
In this section, we will compare the expressiveness of $\SRE$s and rules
against the expressiveness of \textit{regex formulas} ($\RGX$) as defined
in~\cite{FKRV15}. A $\SRE$ $\varphi$ and a $\RGX$ $\gamma$ are said to be
\emph{equivalent} if and only if $\sem{\varphi} = \sem{\gamma}$.

We say that a regex formula $\gamma$ is \textit{plain} if $\gamma$
can be derived using the following grammar.
\begin{equation*}
  R \Coloneqq \emptyset \mid \epsilon \mid R \vee R \mid
       R \cdot R \mid R^{*} \mid x\{\Sigma^{*}\}
\end{equation*}

\begin{lemma}\label{lemma:sre-rgx}
  The class of \emph{functional} $\SRE$s and the class of \emph{plain} $\RGX$s
  are equivalent.
\end{lemma}

\begin{proof}
  We may transform a $\SRE$ $\varphi$ into an equivalent $\RGX$ $\gamma$ by
  replacing $/$ with $\cdot$, $+$ with $\vee$ and $x$ with $x\{\Sigma^{*}\}$
  for every variable $x \in \VV$. Since $\varphi$ is \emph{functional}, $\gamma$
  will also be \emph{functional} and thus a $\RGX$. Since the $\RGX$s are
  \emph{plain}, the reverse transformation will be well defined. It is clear
  that this will take polynomial time and produce polynomial size expressions in
  both directions.
\end{proof}

A \emph{path} $\RGX$ is a formula that can be derived using the following
grammar with $E$ as the \emph{start symbol}.
\begin{align*}
  E &\Coloneqq x\{E\},\ x \in \VV \mid (E \cdot E) \mid R\\
  R &\Coloneqq w,\ w \in (\Sigma \cup \{\epsilon\}) \mid (R \cdot R) \mid
      (R \vee R) \mid {(R)}^{*}
\end{align*}
It is easy to see that \emph{path} $\RGX$ are equivalent to \emph{vstk-path}
automata, since having disjunction at a variable level would require having
multiple paths in the automata.

Similarly, a \emph{path} $\SRE$ is an expression that can be derived from the
following grammar with $E$ as the \emph{start symbol}.
\begin{align*}
  E &\Coloneqq x,\ x \in \VV \mid (E / E) \mid R\\
  R &\Coloneqq w,\ w \in (\Sigma \cup \{\epsilon\}) \mid (R / R) \mid
      (R + R) \mid {(R)}^{*}
\end{align*}

\begin{lemma}\label{lemma:tlstar-rgxnotcup}
  The class of \emph{tree-like} rules using only \emph{path} $\SRE$s and the
  class of \emph{path} $\RGX$s are equivalent.
\end{lemma}

\begin{proof}
  Let $\theta = \doc.\varphi_0 \wedge x_1.\varphi_1 \wedge \cdots \wedge
  x_m.\varphi_m$ be the body of a \emph{tree-like} rule where $x_i \in \VV$ and
  $\varphi_i$ are \emph{path} $\SRE$s. We may transform an individual $\SRE$
  $\varphi$ into a $\RGX$ $\gamma$ with the following procedure: (1) replace
  $+$ with $\vee$ and $/$ with $\cdot$; and (2) for each variable $x_i$,
  replace it with:
  \begin{itemize}
    \item $x_i\{\Sigma^{*}\}$, if no \emph{extraction expression} in $\theta$
      has $x_i$ as its left side.
    \item $x_i\{\gamma_i\}$, if $x_i.\varphi_i$ occurs in $\theta$ and
      $\gamma_i$ is the transformation of $\varphi_i$.
  \end{itemize}
  The $\RGX$ $\gamma_0$ obtained by transforming $\varphi_0$ will be equivalent
  to $\theta$. Since $\theta$ is \emph{tree-like}, the procedure will always
  terminate. It is easy to see that since all $\varphi_i$ are \emph{path}
  $\SRE$s, $\gamma_0$ will be a \emph{path} $\RGX$. The path structure assures
  that each replacement will be made at most once, which implies that the
  transformation will take polynomial time and produce polynomial size
  expressions.

  The inverse transformation can be carried out in a similar fashion: given a
  \emph{path} $\RGX$ $\gamma$ we (1) replace the operators; (2) for each
  variable $x_i\{\gamma_i\}$ we replace it with $x_i$ and add the
  \emph{extraction expression} $x_i.\varphi_i$ where $\varphi_i$ is the
  transformation of $\gamma_i$; and (3) finally add the expression
  $\doc.\varphi$ where $\varphi$ is the result of the transformation. Since
  $\gamma$ is \emph{functional} and does not contain disjunctions among
  variables (its a \emph{path} $\RGX$) each mentioned variable will appear only
  once, and the resulting rule will be \emph{simple}. The tree structure will
  be given by the nested organization of $\RGX$s. As in the other direction it
  is easy to see that this will generate \emph{path} $\SRE$s. It is also
  apparent that the transformation will take polynomial time and produce
  polynomial size expressions.
\end{proof}

For \emph{tree-like} rules using general \(\SRE\)s, the following can be proven.

\begin{lemma}\label{lemma:tl-rgx}
  Every \emph{tree-like} expression can be transformed into an equivalent
  \(\RGX\).
\end{lemma}

\begin{proof}
  We follow the same procedure from Lemma~\ref{lemma:tlstar-rgxnotcup}, with the
  difference that in this case variables might repeat multiple times in the
  \(\SRE\) (through the use of variable-level disjunctions). The resulting
  \(\RGX\) will still be valid, but might be of exponential size, because each
  time a variable is replaced the expression might grow by a factor proportional
  to the size of the rule.
\end{proof}

Now we will show that \emph{tree-like} rules are not sufficient for capturing
$\RGX$s. This is because rules, as $\RGX$, are \emph{hierarchical}, but in a
stronger sense.

\begin{proposition}
  There is a $\RGX$ for which there is no equivalent single rule.
\end{proposition}

\begin{proof}
  Consider the following \RGX{} formula.
  \begin{equation*}
    \gamma = \Sigma^{*} \cdot (x\{y\{\Sigma^{*}\}\cdot a\} \vee
    y\{x\{\Sigma^{*}\cdot a\}\}) \cdot \Sigma^{*}
  \end{equation*}
  This formula can not be expressed by a single rule. To see why, let $\theta$
  be a rule using variables $\VV$. Let $\preceq_{\theta}$ be a binary relation
  over $\VV$ such that $x \preceq_{\theta} y$ if there is a path from $x$ to $y$
  in $G_{\theta}$. Notice that if $x \preceq_{\theta} y$ then every valuation
  $\nu$ that satisfies $\theta$ must have $\nu(x) \sqsubseteq \nu(y)$.

  Therefore, given a rule $\theta$, variables $x, y$ and satisfying valuations
  $\nu_1, \nu_2$ for $\theta$, it's impossible to have $\nu_1(x) \sqsubsetneq
  \nu_1(y)$ and $\nu_2(y) \sqsubsetneq \nu_2(x)$ simultaneously, which is
  certainly possible for $\gamma$.
\end{proof}

A \emph{ruleset} is defined as an \emph{annotation program} with the following
restrictions: (1) rules have no body predicates; and (2) all rules have a
common annotation as head. Naturally, we define \emph{tree-like rulesets} as
those \emph{rulesets} comprised of \emph{tree-like} rules.

\begin{lemma}\label{lemma:utlstar-rgx}
  \emph{Tree-like rulesets} and \(\RGX\) are equivalent.
\end{lemma}

\begin{proof}
  As proved in~\cite{FKRV15}, \(\RGX \equiv \VAStk \equiv \PUStk\). Since
  \emph{path} \(\RGX\)s are equivalent to vstk-paths, then \(\PUStk\) is
  equivalent to the disjunction of \emph{path} \(\RGX\)s. Therefore, we may
  transform a \(\RGX\) into a \emph{tree-like ruleset} using this fact and
  Lemma~\ref{lemma:tlstar-rgxnotcup}. The resulting \emph{tree-like ruleset} is
  going to be of exponential size with respect to the staring \(\RGX\), because
  the transformation from vstk-automata to vstk-path union causes an exponential
  blow up in size.

  We transform a \emph{tree-like ruleset} into a \(\RGX\) by applying
  Lemma~\ref{lemma:tl-rgx} to each rule individually and then joining the
  results with disjunctions. As in that case, the resulting expression might be
  of exponential size.
\end{proof}

Now we will consider \emph{dag-like} rules. As shown before, these are
equivalent to general rules, since cycles can be eliminated by rule rewriting.

\begin{lemma}\label{lemma:rule-dag}
  For every rule there is an equivalent \emph{dag-like} rule. The
  transformation takes polynomial time and produces polynomial size expressions
  in both directions.
\end{lemma}

\francisco{That proof should be here, perhaps?}

Now we show that under a reasonable condition, \emph{dag-like} and
\emph{tree-like} rules are equally expressive. Given a rule \(\theta\), we say
that a variable \(x\) is \emph{trivial} if every document \(d\) and every
assignment \(\nu\) that satisfies \(\theta\) makes \(d(\nu(x)) = \epsilon\).

\begin{lemma}
  When restricting to non-trivial variables, the class of \emph{dag-like} rules
  and the class of \emph{tree-like} rules are equivalent.
\end{lemma}

\begin{proof}
  As explained in Lemma~\ref{lemma:rule-dag}, every variable that can be
  reached from a root through two distinct paths will be given empty content by
  every satisfying assignment and, thus, will be trivial. Therefore every
  variable must be reachable from a root through at most one path, which means
  that the rule will be \emph{tree-like}.
\end{proof}

Nonetheless, we show that even when considering trivial variables, \(\RGX\) can
express \emph{dag-like} rules.

\begin{lemma}\label{lemma:dag-rgx}
  Every \emph{dag-like} rule can be transformed into an equivalent \(\RGX\).
\end{lemma}

\begin{proof}
  As shown before, we only need to consider the ``minimal'' undirected cycles,
  since the rule may be rewritten to remove the rest. To transform rule
  \(\theta\), we apply the same procedure from Lemma~\ref{lemma:tl-rgx}, but
  now, the resulting \(\RGX\) \(\gamma\) might not be functional. In order to
  make \(\gamma\) functional, we can first distribute the disjunction operators
  to obtain a formula \(\gamma' = \bigvee_{1 \leq i \leq k} \gamma'_i\) where
  each \(\gamma'_i\) is free of disjunctions (this might produce an exponential
  blow up in size). Then, in each disjunct, for each repeated variable \(x\),
  make the content of everything between two appearances of \(x\) empty and
  remove all but one of the appearances (has to be consistently chosen in each
  disjunct). If the content can not be made empty, then remove the disjunct
  altogether.

  The resulting \(\RGX\) will be functional and equivalent to \(\theta\). The
  result is going to be of double exponential size with respect to \(\theta\).
\end{proof}

We conclude by showing that general \emph{rulesets} and \(\RGX\)s are equally
expressive.

\begin{theorem}
  \emph{Rulesets} and \(\RGX\) are equivalent. Furthermore, a \emph{ruleset} can
  be transformed into an equivalent \(\RGX\) in \(\TWOEXPTIME\) with a double
  exponential increase in size, and a \(\RGX\) can be transformed into an
  equivalent \emph{ruleset} in \(\EXPTIME\) with an exponential increase in
  size.
\end{theorem}

\begin{proof}
  The proof follows easily from Lemma~\ref{lemma:dag-rgx} and
  Lemma~\ref{lemma:utlstar-rgx}.
\end{proof}

==> Expressiveness-of-RGX.tex <==
% Comparison of Span Regular Expressions vs Regex Formulas.

%\section{Expressiveness of IE languages}\label{sec:expr}
\section{Rules for extracting incomplete data}\label{sec:expr}

In Section \ref{sec-unifying} we defined a theoretical framework for extracting incomplete information. As shown there, \RGX\ formulas of \cite{FKRV15} strictly subsume \SRGX\ of \cite{AMRV16}. However, the approach of \cite{AMRV16} also allows combining \SRGX\ formulas into Datalog-like rules. Therefore, in this section we study the exact connection between the two formalisms in the setting of incomplete information. We start by redefining the rules of~\cite{AMRV16} to allow incomplete data, and then show that, in general, rules are incomparable to \RGX. We also study how a subclass of rules, called simple rules, can be simplified by removing cycles to then show that \RGX\ formulas are equivalent to unions of simple rules.

%, starting from simple rules based on span regular expressions.
%\SRGX, and moving up to the comparison of datalog-like rule language for \SRGX, and its relation with \RGX\ algebras, and different automata models for the two languages.

\subsection{The semantics of rules}
Regex formulas allow the user to specify the shape of the span captured by 
some variable using an expression of the form $x\{\gamma\}$. For example, 
if we wanted to say that the string corresponding to the span captured by the
variable $x$ belongs to the regular language $R$, we would write $x\{R\}$.
As we have seen in the previous section, this immediately makes \RGX\ 
formulas more expressive than \SRGX\ formulas, since the latter cannot constrain 
the shape of the span captured by a variable. So, how can one specify that a
span captured by a variable inside a \SRGX\ formula has a specific shape? 

%A natural approach to solve this issue allows joining \SRGX\ formulas using 
%a rule-like syntax \cite{AMRV16}. For instance, to specify that the content of the spans captured by 
%the variable $x$ belongs to a language in the intersection of two regular expressions $R_1$ and $R_2$,
%we can now write  $x.R_1  \wedge x.R_2$. Of course, since regular languages 
%are closed under intersection, it is also possible to express this property using
%\RGX, however, the resulting expression will generally be less intuitive 
%than the simple rule above. One can see that the two approaches to information
%extraction have slightly different design philosophies: on the one hand, we have 
%the concise syntax of \RGX, and on the other hand we have a more visual approach
%which combines \SRGX\ formulas into rules. In this section we explore how these two
%approaches compare in terms of expressive power.

%A natural
%approach to solve this issue allows joining \SRGX\ formulas using 
%a rule-like syntax \cite{AMRV16}. For instance, to specify that the content of the spans captured by 
%the variable $x$ belongs to a language in the intersection of two regular expressions $R_1$ and $R_2$,
%we can now write  $x.R_1  \wedge x.R_2$. Of course, since regular languages 
%are closed under intersection, it is also possible to express this property using
%\RGX, however, the resulting expression will generally be less intuitive 
%than the simple rule above. One can see that the two approaches to information
%extraction have slightly different design philosophies: on the one hand, we have 
%the concise syntax of \RGX, and on the other hand we have a more visual approach
%which combines \SRGX\ formulas into rules. In this section we explore how these two
%approaches compare in terms of expressive power.

\smallskip

A natural approach to solve this issue allows joining \SRGX\ formulas using 
a rule-like syntax as proposed in \cite{AMRV16}.
To do this, we propose a rule-based language for extracting incomplete
information from documents that is based on \SRGX\ formulas. 
Specifically, in our language 
we will allow two types of formulas: $R$ and $x.R$, where
$R$ is a \SRGX\ formula and $x$ a variable. The former is meant to be evaluated over the entire document,
while the latter applies to the span captured by the variable $x$. The semantics of the
extraction formula $R$  over a document $d$ is defined as above, and for $x.R$ as follows:
$$
  \semd{x.R} \ = \ \{ \mu \mid \exists s. (s,\mu)\in \sempd{x\{R\}} \}.
$$
We can now define rules for extracting information from a document as conjunctions
of extraction formulas. Formally,
 an \emph{extraction rule} is an expression of the form:
\begin{equation*} \label{eq-ann-rule}
\varphi = \varphi_0 \wedge x_1.\varphi_1 \wedge \cdots \wedge x_m.\varphi_m \tag{\dag}
\end{equation*}
where $m \geq 0$, all $\varphi_i$ are \SRGX\ formulas, and $x_i$ are variables\footnote{For simplicity we assume that there is only one formula applying to the entire document; namely $\varphi_0$. It is straightforward to extend the definitions below to include multiple formulas of this form.}. Extraction rules typically have an implication symbol and a \emph{head predicate}, which we will omit because it does not affect the analysis performed in this paper.

While \cite{AMRV16} has a simple definition of the semantics of extraction rules, lifting this definition to the domain of mappings requires us to account for nondeterminism of our expressions. What we mean by this is perhaps best captured by the rule $(x \vee y) \wedge x.(ab^*) \wedge y.(ba^*)$, where we first choose which variable is going to be mapped to the entire document, and then we need to satisfy its respective constraint. For instance, if $x$ is matched to the document, we want it to conform to the regular expression $ab^*$; however, in this case we do not really care about the content of $y$, so we should leave our mapping undefined on this variable.

%The second challenge, ``ghost variables", refer to variables which are not linked to a specific part of a document, but can be assigned arbitrary spans. For instance, in a rule $\Sigma^* \wedge x.ab^*$, the variable $x$ does not really give us any information about the document itself, since it talks about arbitrary spans. What we really want is to link it to the rule applying to the entire document somehow; be it so that it appears in this formula itself (e.g. in $\Sigma^*x\Sigma^* \wedge x.ab^*$), or can reach it through other variables (e.g. in $\Sigma^*y\Sigma^* \wedge y.x \wedge x.ab^*$). We account for such behaviour as follows.

Formally, we define when a rule of the form (\ref{eq-ann-rule}) is satisfied by a tuple of mappings $\overline{\mu}=(\mu_0,\mu_1,\ldots ,\mu_m)$. To avoid the problem mentioned above, we need the concept of {\em instantiated variables} in our tuple of mappings. 
For a rule $\varphi$ of the form (\ref{eq-ann-rule}) and a tuple of mappings $\overline{\mu}=(\mu_0,\mu_1,\ldots ,\mu_m)$ we define the set of \emph{instantiated variables}, denoted by $\ivar(\varphi,\overline{\mu})$ as the minimum set such that $dom(\mu_0)\subseteq \ivar(\varphi,\overline{\mu})$ and if $x_i\in \ivar(\varphi,\overline{\mu})$, then 
$dom(\mu_i)\subseteq \ivar(\varphi,\overline{\mu})$.
Intuitively, we want to put in $\ivar(\varphi,\overline{\mu})$ only the variables which are used in nondeterministic choices made by $\varphi$ and $\overline{\mu}$. For instance, in the rule $(x \vee y) \wedge x.(ab^*) \wedge y.(ba^*)$, if we decide that $x$ should be matched to our document, then we will not assign a value to the variable $y$ and vice versa. We now define that a tuple of mappings $\overline{\mu}=(\mu_0,\mu_1,\ldots ,\mu_m)$ satisfies $\varphi$ over a document $d$, denoted by $\overline{\mu}\models_d \varphi$, if the following three conditions hold: (1) $\mu_0\in \semd{\varphi_0}$; (2) $\mu_i \in \semd{x_i.\varphi_i}$  whenever $x_i\in \ivar(\varphi,\overline{\mu})$ and $\mu_i = \emptyset$ otherwise; and (3) $\mu_i\sim \mu_j$ for all $i,j$.
%\begin{itemize}\itemsep=0pt
%\item[-] $\mu_0\in \semd{\varphi_0}$;
%\item[-] If $x_i\in \ivar(\varphi,\overline{\mu})$ then $\mu_i \in \semd{x_i.\varphi_i}$;
%\item[-] If $x_i\notin \ivar(\varphi,\overline{\mu})$ then $\mu_i = \emptyset$; and
%\item[-] $\mu_i\sim \mu_j$ for all $i,j$.
%\end{itemize}
Here the last condition will allow us to ``join'' all the mappings capturing each subformula $\varphi_i$ into one. The problem with nondeterminism is handled by condition (2), since we force all instantiated variables to take a value, and the non-instantiated ones to be undefined. Finally, condition (1) starts from $\varphi_0$ which refers to the entire document and serves as a ``root'' for our mappings.


We can now define the semantics of an extraction rule $\varphi$ over a document
$d$ as follows:
$$
  \semd{\varphi} \ = \ \{ \mu \mid \exists \overline{\mu} \text{ such that } \overline{\mu}\models_d \varphi \text{ and } \mu = \bigcup_i \mu_i \},
$$
where $\bigcup_i \mu_i$ denotes the mapping defined as the union of all $\mu_i$.

Extraction rules allow us to define complex conditions about the spans we wish to extract. For instance, if we wanted to extract all spans whose content is a word belonging to (ordinary) regular expressions $R_1$ and $R_2$ at the same time, we could use the rule $\Sigma^*\cdot x \cdot \Sigma^* \wedge x.R_1 \wedge x.R_2.$ More importantly, using extraction rules, we can now define valuations which cannot be defined using \RGX, since they can define mappings which are not hierarchical. For instance, the rule $x\wedge x.ayaa \wedge x.aaza$ is one such rule, since it makes $y$ and $z$ overlap on the document $aaaaa$.
%To see this, consider a rule of the form $x \wedge x.a\cdot y \wedge x.a\cdot z$,
%which defines valuations where both $y$ and $z$ are part of the document after the initial letter $a$.
%Clearly, such a rule cannot be defined using \RGX, since the spans assigned to $y$ and $z$ always have
%to be the same. 
In some sense, the ability of rules to use conjunctions of variables makes them
more powerful than \RGX\ formulas. % in some cases.
On the other hand, the ability of \RGX\ formulas to use
disjunction of variables poses similar problems for \SRGX. 
Here one separating example is the \RGX\ formula $(a \cdot
x\{b\}) \vee (b \cdot x\{a\})$. 
%Therefore, we have the following:

\begin{theorem} \label{prop-rgx-rules}
Extraction rules and \RGX\ are incomparable in terms of the expressive power.
\end{theorem}
In light of this result, we study next which fragments of the two languages are equivalent.
%We address this question next

\subsection{Eliminating cycles from rules}

In order to capture \RGX\ formulas, we first need to prune the class of rules we allow, since already a single rule can express properties beyond the reach of \RGX. 
As we have seen, the capability of an extraction rule to use conjunctions of the same variable multiple times already takes them outside of the reach of \RGX. Therefore, the most general class of rules we will consider disallows that type of behaviour. We call such rules {\em simple rules}. Formally, an extraction rule $\varphi$ of the form (\ref{eq-ann-rule}) is {\em simple}, if all $x_i$ are pairwise distinct. 
From now on, we assume that all classes of rules considered in this section are simple. 

Another feature that makes rules different
from \RGX\ is their ability to enforce cyclic behaviour through expressions of the form $x.y \wedge y.ax$.
A natural way to circumvent this shortcoming is to force the rules to have an acyclic structure. 
In fact, this kind of restriction was already considered in \cite{AMRV16}, as it allows faster evaluation than general rules.
Therefore, a natural question at this point is if the capability of rules to define cycles is really useful, or if they can be removed.
We answer now the question whether cycles can be eliminated from rules, and somewhat surprisingly show that, while generally not possible, in the case of rules defined by functional \SRGX\ this is indeed true.

In order to study the cyclic behaviour of rules, we first need to explain how each rule can be viewed as a graph.
To each extraction rule $\varphi=\varphi_0 \wedge x_1.\varphi_1 \wedge \cdots \wedge x_m.\varphi_m$ we associate a graph $G_\varphi$ defined as follows. The set of nodes of $G_{\varphi}$ contains all the variables $x_1,\ldots ,x_m$ plus one special node labelled $\texttt{doc}$ corresponding
to the formula $\varphi_0$.
There exists an edge $(x, y)$ between two variables in $G_{\varphi}$ if, and only if, there is an
\emph{extraction formula} $x.R$ in $\varphi$ such that $y$ occurs in
$R$. Furthermore, if the variable $x$ occurs in the formula $\varphi_0$, we add an edge $(\texttt{doc},x)$ to $G_\varphi$.
Then we say that a simple rule $\varphi$ is {\em dag-like}, if the graph $G_\varphi$ contains no cycles, and \emph{tree-like} if $G_{\varphi}$ is a tree rooted at $\texttt{doc}$. 

To answer the question whether cycles can be eliminated from rules, let us consider most general case; namely, simple rules over full \RGX. It is straightforward to see that in a rule of the form $(x \vee y) \wedge x.(y \vee \Sigma^*) \wedge y.(x \vee \Sigma^*)$, the cycle formed by $x$ and $y$ cannot be broken and the rule cannot be rewritten as a single dag-like rule. The main obstacle here is the fact that in each part of the rule we make a nondeterministic choice which can then affect the value of all the variables.
However, there is one important class of expressions, which would prohibit our rules to define properties such as the one above; that is, functional \SRGX. 
%The notion of functionality, first introduced in \cite{FKRV15}, was shown to be crucial for having a well-behaved fragment of \RGX\ formulas, and it also has a profound effect on complexity of formula evaluation, since it brings it down from $\NP$-hard to tractable (see Section \ref{sec:eval}). As defined previously, functional formulas force that the variables used on the two sides of a disjunction are always the same, and furthermore, require concatenated expressions to share no variables (thus also forcing the star operator to be allowed only over variable-free formulas). 
In the next result, we show that in the case of functional rules (i.e.\ rules defined by functional \SRGX) cycles can always be removed, and in fact, converting a simple functional rule into a dag-like rule takes only polynomial time.

\begin{theorem}\label{thm:simple_to_dag}
	For every simple rule that is functional there is an equivalent (functional) dag-like rule. Moreover, we can obtain the equivalent rule in polynomial time.
\end{theorem}

It is remarkable that the algorithm for removing cycles runs in polynomial time and, furthermore, it produces a single rule. 
We think that this result is interesting in its own right and potentially useful in other contexts regarding the use of rules in information extraction.

\subsection{Unions of simple rules capture RGX}

We now know that cycles can be eliminated from functional rules, but is there any way to removes cycles from rules that are non-functional? Moreover, can we go even further from dag-like rules, and convert each rule into a tree-like rule? 
Unfortunately, one can easy show that all these questions have a negative answer since non-functional cyclic rules, and even functional dag-like rules, have the ability to express some sort of disjunction.
For this reason, we introduce here the class of \emph{unions of simple rules} and compare its expressive power with \RGX.  
Formally, {\em union of simple rules} is a set of simple rules $A$. The semantics $\semd{A}$ over a 
document $d$ is defined as all mapping $\mu$ over $d$ such that $\mu \in \semd{\varphi}$ for some $\varphi\in A$.

We start by extending our results for removing cycles from functional to non-functional rules. 
As it turns out, although functional and non-functional rules are not equivalent, every non-functional simple rule can in fact be expressed as a union of functional rules.
Then, by combining this fact with Theorem~\ref{thm:simple_to_dag} one can show that each non-functional rule can be made acyclic by transforming it to a  \emph{union of dag-like rules}. 

\begin{proposition}\label{prop:nonfunc}
	Every simple rule is equivalent to a union of functional dag-like rules. 
\end{proposition}

Now that the connection with union of acyclic rules is settled, our next step is to understand when dag-like rules can be defined by \RGX\ formulas and, moreover, when can they be converted into tree-like rules.
First, observe that a functional \RGX\ formula is always satisfiable; namely, there is always a document on which there is an assignment satisfying this formula. Similarly, every functional tree-like rule is also satisfiable. On the other hand, the functional simple rule $x\wedge x.y \wedge y.ax$ is clearly not satisfiable, since it forces $x$ and $y$ to be equal and different at the same time. Therefore, to link rules with \RGX, we should consider only the satisfiable ones.

\begin{proposition}\label{thm:dag_to_tree}
	Every dag-like rule that is satisfiable is equivalent to a union of functional tree-like rules.
\end{proposition}

The idea of the proof here is similar to the cycle elimination procedure of Theorem \ref{thm:simple_to_dag}, but this time considering undirected cycles. One can show that eliminating undirected cycles results in a double exponential number of tree-like rules. In case that the rule was not satisfiable, our algorithm will simply abort.

%The idea of the proof here is similar to the cycle elimination procedure above, but this time we need to consider undirected cycles, or more precisely, we consider all pairs of nodes which are linked by two or more distinct paths. Such undirected cycles are then removed based on whether the final node is coloured green or red. Furthermore, one can show that eliminating undirected cycles results in a double exponential number of tree-like rules. In case that the rule was not satisfiable, our algorithm will simply abort.

With this at hand, we can now describe the relationship between unions of simple rules and \RGX. Indeed, a union of simple rules is equivalent to a  union of dag-like rules by Proposition~\ref{prop:nonfunc} and this union is equivalent to a union of functional tree-like rules by Proposition~\ref{thm:dag_to_tree} (if some dag-like rule is not satisfiable, we just output an unsatisfiable non-fuctional RGX formula in our algorithm from Proposition \ref{thm:dag_to_tree}). 
Then one can easily see that any functional tree-like rule $\varphi$ is equivalent to a $\RGX$ formula given that each (singleton) formula $x.R$ in $\varphi$ can be removed by composing the tree structure recursively with formulas of the form $x\{R\}$.
Conversely, one can show that each $\RGX$ formula can be defined as a union of simple rules.

\begin{theorem}\label{thm:rgx:simple}
	\RGX\ formulas and unions of simple rules are equivalent. Moreover, every \RGX\
  formula is equivalent to a union of tree-like rules.
\end{theorem}
















\begin{comment}

\newpage
\cristian{OLD SECTION}

\subsection{Union of tree-like rules capture RGX}

%%Of course, a natural question now is which fragments of the two languages are equivalent.
%In order to cover all \RGX\ formulas, we will show how unions of rules can be used to simulate the disjunction
%of variables. However, for this we also need to prune the class of rules we allow,
%since already a single rule can express properties beyond the reach of \RGX. As we have seen, 
%allowing conjunction of the same variable is problematic for \RGX. This leads us to the class
%of simple rules. An extraction rule is {\em simple}, if (1) it uses an expression formula {\it not} of 
%the form $x.R$ at most once; and (2) every variable appears at most once in an expression of the form
%$x.R$. However, even simple rules can go beyond \RGX.
%
%\begin{lemma}
%There is a simple extraction rule with no equivalent \RGX\ formula.
%\end{lemma}
%
%The result here is due to the fact that simple rules still allow ``cyclic" definitions such as $x.y \wedge y.ax$,
%which can make them un-satisfiable: a property which they do not share with \RGX. 
%%
%%MOVE TO DAG-LIKE 
%%
%%\bigskip
%%
%%HERE COMES THE TREE-LIKE STUFF
%%
%%
%A way around this is to prohibit
%such behaviour by forcing the rules to have a tree-like structure. In fact, this class of extraction
%rules was alreadyfirst need to define considered in \cite{AMRV16}, as it allows faster evaluation than the class of all rules.
%In order to define the class of {\em tree-like rules}, we need to explain how each rule can be viewed as a graph.

%Of course, a natural question now is which fragments of the two languages are equivalent.

In order to express all \RGX\ formulas, we will show how unions of rules can be used to simulate the disjunction
of variables. However, for this we also need to prune the class of rules we allow,
since already a single rule can express properties beyond the reach of \RGX. As we have seen, 
allowing conjunctions of the same variable is problematic for \RGX. Another thing that makes rules different
from \RGX\ is their ability to enforce cyclic behaviour through expressions of the form $x.y \wedge y.ax$.
A natural way to circumvent both of these shortcomings is to force the rules to have a tree-like structure. 
In fact, this class of extraction
rules was already considered in \cite{AMRV16}, as it allows faster evaluation than general rules.
In order to define the class of {\em tree-like rules}, we need to explain how each rule can be viewed as a graph.

To each extraction rule $\varphi=\varphi_0 \wedge x_1.\varphi_1 \wedge \cdots \wedge x_m.\varphi_m$ we associate a graph $G_\varphi$ defined as follows. The set of nodes of $G_{\varphi}$ contains all the variables $x_1,\ldots ,x_m$ plus one special node labelled $\texttt{doc}$ corresponding
to the formula $\varphi_0$.
There exists an edge $(x, y)$ between two variables in $G_{\varphi}$ if and only if there is an
\emph{extraction formula} $x.R$ in $\varphi$ such that $y$ occurs in
$R$. Furthermore, if the variable $x$ occurs in the formula $\varphi_0$, we add an edge $(doc,x)$ to $G_\varphi$.
Then we say that $\varphi$ is \emph{tree-like} if (1) every variable $x$ appears at most once on the left-hand side of an expression of the form
$x.R$; and (2) $G_{\varphi}$ is a tree rooted at $\texttt{doc}$. 
%We can now show that the class of tree-like rules is indeed subsumed by \RGX.
%
%\begin{lemma}\label{lemma:tl-rgx}
%  Every \emph{tree-like} rule can be transformed into an equivalent
%  \(\RGX\).
%\end{lemma}

As we know, \RGX\ alone is more expressive than any single rule, but by allowing unions of
tree-like rules, we get a class of extraction rules capturing \RGX\ formulas. Formally,
{\em union of tree-like rules} is a set of tree-like rules $A$. The semantics $\semd{A}$ over a 
document $d$ is defined as all mapping $\mu$ over $d$ such that $\mu \in \semd{\varphi}$ for some $\varphi\in A$.
%\begin{gather*}
%  \semd{A} \ = \ \{ \mu \mid \mu \text{ is a variable assignment over }
%      d\\
%   \hspace{65pt} \text{ such that } \mu \in \semd{\varphi}, \text{ for some } \varphi\in A \}.
%\end{gather*}
With this in hand, we can now better understand the connection between rules and \RGX:

\begin{theorem}\label{lemma:utlstar-rgx}
Unions of tree-like rules are equivalent to \(\RGX\) formulas.
\end{theorem}

%The proof of this theorem relies on the fact that \RGX\ formulas are equivalent
%to unions of functional \RGX\ which do not use disjunctions of (expressions
%containing) variables. The latter can then be easily expressed using a tree-like rule, giving us one direction of the theorem. The other direction follows from Lemma \ref{lemma:tl-rgx} and the fact that \RGX\ formulas are closed under disjunction. Analysing the proof also shows us that the transformation is exponential in both directions.

%The proof of this theorem relies on the fact that \RGX\ formulas are equivalent to 
%variable stack (\VAStk) automata \cite{FKRV15}. Furthermore, \cite{FKRV15} also shows that every
%\VAStk\ automaton can be transformed into a \VAStk\ automaton which consists of disjoint paths
%connecting the starting and the accepting state, also known as path-union automaton, or \PUStk.
%Using this, we can show that every \RGX\ is equivalent to a disjunction of \RGX\ formulas which
%do not use disjunction of (expressions containing) variables, since each such expression can
%be viewed as one path in \PUStk\ automaton. Finally, we show that each \RGX\ not containing
%disjunctions of variables can be defined using a tree-like rule, therefore allowing us to express
%an arbitrary \RGX\ as a union of tree-like rules. The other direction of the theorem follows from 
%Lemma \ref{lemma:tl-rgx} and the fact that \RGX\ formulas are closed under disjunction.


%\smallskip

%Apart from knowing that the classes of \RGX\ formulas and unions of tree-like rules are equivalent, one might also be
%interested in how difficult it is to compute the equivalent expression. Here we can show that to define
%a single tree-like rule one requires an exponential size \RGX\ formula,
%since extraction rule can contain \SRGX\ which repeat the same variable multiple times. 
%On the other hand, defining a \RGX\ by union of tree-like rules requires an exponential number of rules, because to represent
%a \RGX\ using \PUStk\ we might already need exponentially many paths in our automaton.

\subsection{Eliminating cycles from rules}

%WILL INTEGRATE THIS INTO SEC 3.2. AFTERWARDS IF CRISTIAN MAKES ME
%
%The result here is due to the fact that simple rules still allow ``cyclic" definitions such as $x.y \wedge y.ax$,
%which can make them un-satisfiable: a property which they do not share with \RGX. So how can we restrict the class
%of rules in order to prohibit such behaviour? For this, we first need to consider the graph structure of each rule.
%
%To each extraction rule $\varphi$ we associate a graph $G_\varphi$ defined as follows. The
%set of nodes of $G_{\varphi}$ is the set of variables occurring in $\varphi$, and
%there exists an edge $(x, y)$ in $G_{\varphi}$ if and only if there is an
%\emph{extraction formula} $x.R$ in $\varphi$ such that $y$ occurs inside 
%$R$. If the graph $G_\varphi$ contains no cycles, we call the rule $\varphi$ a {\em dag-like} rule,
%since it resembles a directed acyclic graph. It is then not difficult to see that each dag-like
%rule has an equivalent \RGX.
%
%\begin{lemma}\label{lemma:dag-rgx}
%  Every \emph{dag-like} rule can be transformed into an equivalent \(\RGX\).
%\end{lemma} 
%
%What is perhaps more surprising, is the fact that we can rewrite each simple rule into an equivalent dag-like rule; that is,
%we can remove cycles from our rules.


%EMPH ON SAT:
%The example showing that not all simple rules can be expressed as \RGX\ relies on the fact that rules can define cycles in their associated graph and can as such force them to not be satisfiable. This is easily circumvented by going to tree-like rules, but this jump seems rather ad hoc, since it does not answer the question of what happens with simple rules that are satisfiable? What we show in this subsection is that if a simple rule is satisfiable we can remove cycles from it, and that we can then transform it to a union of tree-like rules.

%RULES ONLY, NOT MENTIONING SAT:


%The example showing that not all simple rules can be expressed as \RGX\ relies on the fact that rules can define cycles in their associated graph. This is easily circumvented by going to tree-like rules, but the jump seems rather ad hoc, since there is a more general class of rules which prohibit such behaviour; namely dag-like rules. We call a rule $\varphi$ a {\em dag-like rule}, if the graph $G_\varphi$ contains no cycles. Perhaps surprisingly, one can actually show that each simple rule can be rewritten into a dag-like rule in polynomial time by eliminating the cycles from it. In this subsection we present an algorithm for cycle elimination from rules, and discuss how simple rules are connected to tree-like rules and \RGX.

In the previous subsection we isolated a class of rules whose unions are equivalent to \RGX\ formulas. To do this, we prohibited rules from using conjunctions of the same variable multiple times, and forced them to have a tree-like structure. And while prohibiting arbitrary conjunction was shown to be crucial, we have still not answered if the capability of rules to define cycles is really an obstacle, or if they can be removed. Consider for instance a rule of the form  $x \wedge x.y \wedge y.x$, whose underlying graph is cyclic. This rule is clearly equivalent to $x\wedge x.y$, that requires no cycles in order to express the same property. In this section we consider the question whether cycles can be eliminated from rules, and somewhat surprisingly show that, while generally not possible, in the case when all expressions defining a rule are functional \SRGX\ formulas this is indeed true. %We also discuss how this relates to the difference in expressiveness of different classes of rules.

%as cyclic rules could still be equivalent to \RGX\ formulas in terms of mappings they define. For instance, the rule $x \wedge x.y \wedge y.xz$ is easily seen to be equivalent to the \RGX\ $x\{y\{z\{\varepsilon\}\}\}$. Surprisingly, in this section we show that unions cyclic rule which prohibit arbitrary conjunctions are indeed equivalent to \RGX. We start by showing something even more surprising; namely, that one can eliminate cycles from cyclic rules without losing expressive power. We then show how such acyclic rules are connected to tree-like rules and \RGX. 

Let us formally define the classes of rules we will consider in this section. First, as discussed above, the capability of an extraction rule to use conjunctions of the same variable multiple times already takes them outside of the reach of \RGX. Therefore the most general class of rules we will consider disallows that type of behaviour. We call such rules {\em simple rules}. Formally, an extraction rule $\varphi = \varphi_0 \wedge x_1.\varphi_1 \wedge \cdots \wedge x_m.\varphi_m$ is {\em simple}, if all $x_i$ are pairwise distinct. Note that simple rules can still be ``cyclic" in nature, namely, the graph $G_\varphi$ associated with the rule $\varphi$ can have cycles. We call a rule $\varphi$ {\em dag-like}, if the graph $G_\varphi$ contains no cycles. Furthermore, a rule $\varphi$ is called {\em functional}, if all of the \SRGX\ formulas $\varphi_0, \ldots ,\varphi_m$ are functional \SRGX\ formulas.

To answer the question whether cycles can be eliminated from rules, let us consider most general case; namely, simple rules over full \RGX. It is straightforward to see that in a rule of the form $(x \vee y) \wedge x.(y \vee \Sigma^*) \wedge y.(x \vee \Sigma^*)$, the cycle formed by $x$ and $y$ cannot be broken and the rule cannot be rewritten as a single dag-like rule. The main obstacle here is the fact that in each part of the rule we make a nondeterministic choice which can then affect the value of all the variables.
However, there is one important class of expressions, which would prohibit our rules to define properties such as the one above; that is, functional span regular expressions. The notion of functionality, first introduced in \cite{FKRV15}, was shown to be crucial for having a well-behaved fragment of \RGX\ formulas, and it also has a profound effect on complexity of formula evaluation, since it brings it down from $\NP$-hard to tractable (see Section \ref{sec:eval}). As defined previously, functional formulas force that the variables used on the two sides of a disjunction are always the same, and furthermore, require concatenated expressions to share no variables (thus also forcing the star operator to be allowed only over variable-free formulas). Somewhat surprisingly, we can show that in the case of functional rules cycles can always be removed, and in fact, converting a simple rule that is functional into a dag-like rule takes only polynomial time.

%Take therefore an arbitrary simple rule that is {\em functional}.
%We start by analysing what sort of a value can a mapping assign to the variables which form a cycle.
%For this take any rule $\varphi$ and assume that there is a simple cycle $x_1,\ldots ,x_n$ appearing in $G_\varphi$ and a mapping $\mu$ satisfying $\varphi$. Then the following must hold:
%\begin{enumerate}
%\item {\em All variables in the cycle must be assigned the same value.} This follows from the fact that in a simple rule each edge $(x,y)$ in $G_\varphi$ implies that $\mu(x)$ contains $\mu(y)$.
%\item {\em Every variable reachable from a cycle, but not inside it, must be assigned the empty content.} This follows from the observation above, plus the fact that edges $(x,y)$ and $(x,y)$ in $G_\varphi$ imply that $\mu(y)$ and $\mu(z)$ are disjoint.
%\item {\em If the cycle has a chord, then all the variables inside it must be assigned the empty content.} Here a chord means that we have a path from some $x_i$ to some $x_j$ inside $G_\varphi$ which consists of nodes not belonging to our cycle,  or there is a direct edge between them which is not part of the cycle. In the case there is an intermediate node, we know that it must be assigned $\varepsilon$, therefore $x_j$ and all other nodes in the cycle must be $\varepsilon$ as well. If the edge is direct, then by the definition of a chord, $x_j$ is not a successor of $x_i$ in the cycle, so just as in the previous case, the content of the successor of $x_i$ and the content of $x_j$ must be disjoint and equal, which is only possible if they are $\varepsilon$.
%\end{enumerate}
%
%The procedure for eliminating cycles from simple rules is based on the following colouring scheme for a graph
%$G_{\varphi}$ associated with the rule $\varphi$. Let $\varphi$ be an extraction rule with variables $x_1,\ldots x_n$. We will
%colour a node $x_i$ {\em black} if:
%\begin{itemize}
%\item $x_i.\varphi_i$ appears in $\varphi$ and $\varphi_i$ has at least one symbol of the alphabet which is not under the star operator $*$; that is, the variable $x_i$ must contain at least one occurrence of an alphabet letter.
%\end{itemize}
%We then paint the graph by assigning the colour {\em red} to all black nodes, and all nodes which can reach a black node. All other nodes are coloured {\em green}. It is clear that this procedure can be carried out in polynomial time, since reachability takes only polynomial time. Note that in a black node coming from a conjunct of the form $x_i.\varphi_i$, the content of each variable appearing in $\varphi_i$ must be {\em strictly} contained in the content of the variable $x_i$, because $\varphi_i$ is functional. Also note that each cycle has to be coloured using the same color.
%
%If we now have a simple cycle $x_1,\ldots ,x_n$ we can eliminate it by considering its color:
%\begin{itemize}
%\item {\em If the cycle is coloured red, then the rule is not satisfiable, so we can replace it by an arbitrary unsatisfiable dag-like rule.} We have two cases here. First, if a rule contains a black node, then the content of its successor must be strictly contained inside its own content, which cannot happen by the analysis above. Second, if a node $x$ in the cycle can reach some black node not inside the cycle, then its content must be different from $\varepsilon$ (because the content of the black node is different from it), but then $x$ must also strictly contain the content of its successor in the cycle, which is a contradiction by the above analysis.
%\item {\em If the cycle is green we can simplify it using an auxiliary variable.} Let $u_1, \ldots, u_m$ be the variables that are not
%  part of the cycle and for which there is an edge $(u_i, x_1)$. Let $y_1,
%  \ldots, y_l$ be the variables that are not part of the cycle and are reachable
%  from some $x_i$ (they must have empty content, as proved before). We then add an auxiliary variable $w$ and and edge from it to $x_1$. Each expression associated with some $u_i$ is changed so that it uses $w$ instead of $x_1$, and all expression associated with some $y_i$ are changed to $y_i.\varepsilon$. Next, an expression $x_i.\varphi_i$ is changed to  $x_i.\varphi_i'$, where $\varphi_i'$ maintains the ordering of variables in $\varphi_i$ that are not under a star operator and removes all other letters or starred subexpressions, for $i<n$. For $x_n$, we replace the occurrence of $x_1$ by $\Sigma^*$. This yields an equivalent \emph{simple} rule without the mentioned cycle.
%\end{itemize}
%
%As an example of how the rewriting above works, consider the rule $x.y \wedge y.z \wedge z.ux.$
%This rule can be rewritten to $w.x \wedge x.y \wedge y.z \wedge z.u \wedge u.\varepsilon$.
%
%\domagoj{We should say where is the functionality of rules used!}
%
%Of course, here we explained only how a single cycle can be removed, but how do we transform a rule with multiple cycles in its graph? For this we start by identifying the strongly connected components of our graph $G_\varphi$. Each component can then be either: (a) a single node, (b) a simple cycle, or (c) a simple cycle with additional edges. In the latter two cases, if any component is coloured red, we know that the rule is unsatisfiable, so we can replace it by an arbitrary unsatisfiable dag-like rule. In the case they are coloured green, we can deploy the procedure above to remove the cycles, taking care that in the case (b) our variables can take an arbitrary, but always equal value, while in the case (c) they must be equal to the empty content. In both cases, all the variables reachable from the component are made $\varepsilon$. Since strongly connected components can be computed in polynomial time, we obtain the following.

\begin{theorem}\label{thm:simple_to_dag}
For every simple rule that is functional there is an equivalent (functional) dag-like rule. Moreover, we can obtain the equivalent rule in polynomial time.
\end{theorem}

We now know that cycles can be eliminated from functional rules, but is there any way to simplify rules that are not functional? As it turns out, although functional and non-functional rules are not equivalent, every non-functional simple rule can in fact be expressed as a union of functional rules. 

\begin{proposition}\label{prop:nonfunc}
Every non-functional simple rule is equivalent to a union of functional simple rules.
\end{proposition}

To see this, observe first that every non-functional \SRGX\ formula can be expressed as a (potentially exponentially big) union of functional \SRGX\ formulas (Theorem~\ref{lemma:utlstar-rgx}). Therefore, each non-functional rule $\varphi_0 \wedge x_1.\varphi_1 \wedge \cdots \wedge x_m.\varphi_m$ can be rewritten into a rule whose formulas $\varphi_i$ are unions of functional \SRGX. Now each such rule can be transformed into a union of functional rules by taking all the possible disjunctions (of which there will generally be exponentially many).



\subsection{Regex vs. rules}

One final thing we would like to determine is the connection of the more general classes of simple and dag-like rules to \RGX. We will start by considering functional rules and comparing them to functional \RGX\ formulas. As shown in Theorem~\ref{lemma:utlstar-rgx}, unions of tree-like rules are equivalent to \RGX. It is straightforward to see that this is still true when we consider functional rules and \RGX. Therefore to connect functional rules which are not necessarily tree-like to \RGX, we will show how and when can they be viewed as tree-like.

First, observe that a functional \RGX\ formula is always satisfiable; namely, there is always a document on which there is an assignment satisfying this formula. Similarly, every functional tree-like rule is also satisfiable. On the other hand, the functional simple rule $x\wedge x.y \wedge y.ax$ is clearly not satisfiable, since it forces $x$ and $y$ to be equal and different at the same time. Therefore, to link functional rules with \RGX, we need to consider only the satisfiable ones. As we know that each functional simple rule has an equivalent dag-like rule (Theorem XXX), we start there.


\begin{theorem}\label{thm:dag_to_tree}
Every functional dag-like rule that is satisfiable  is equivalent to a union of functional tree-like rules.
\end{theorem}

The idea of the proof here is similar to the cycle elimination procedure of Theorem \ref{thm:simple_to_dag}, but this time considering undirected cycles. One can show that eliminating undirected cycles results in a double exponential number of tree-like rules. In case that the rule was not satisfiable, our algorithm will simply abort.

%The idea of the proof here is similar to the cycle elimination procedure above, but this time we need to consider undirected cycles, or more precisely, we consider all pairs of nodes which are linked by two or more distinct paths. Such undirected cycles are then removed based on whether the final node is coloured green or red. Furthermore, one can show that eliminating undirected cycles results in a double exponential number of tree-like rules. In case that the rule was not satisfiable, our algorithm will simply abort.

With this at hand, we can now also describe the relationship between functional simple rules and \RGX.

\begin{theorem}\label{thm:simple_to_rgx}
The class of functional \RGX\ formulas is equivalent to unions of satisfiable functional simple rules.
\end{theorem}

As we have shown, simple rules are equivalent to dag-like rules in the functional case. It is not difficult to see that each functional dag-like rule has an equivalent functional \RGX. On the other hand, we have also shown that each satisfiable functional dag-like rule can be expressed as a union of functional tree-like rules. And while a single dag-like rule is not enough to express an arbitrary \RGX\, similarly as in the case of tree-like rules, we can show that their unions can.

%Whether the same holds in the case of non functional rules is not entirely clear, as general \RGX\ formulas can be unsatisfiable. We conjecture that in this case general \RGX\ formulas are equivalent in expressive power to unions of simple rules.

Since we know by Theorem~\ref{lemma:utlstar-rgx} and comments below that each \RGX\ is equivalent to a union of functional \RGX\ formulas (with the union being empty when \RGX\ is not satisfiable), we can also get a more general result.

\begin{theorem}\label{thm:rgx:simple}
\RGX\ formulas are equivalent to unions of functional simple rules.
\end{theorem}



%\subsection{Extraction programs}
%
%Using unions is only a small extension to extraction rules. To harness the full power of the language based on such rules, the authors in \cite{AMRV16} allow combining them using datalog-like programs. In this subsection we explore how such a language compares to automata models for \RGX\ formulas and their algebraic closures.
%
%In order to define datalog programs based on extraction rules, we first extend rules with the ability to use arbitrary arity predicates. For this, let $\Gamma$ be a finite alphabet of predicates (of not necessarily same arity), which is disjoint from the alphabet $\Sigma$ and the set of variables $\VV$. 
% A \emph{general extraction rule} is an expression of the form:
%\begin{equation*} \label{eq-ann-prog}
%  \varphi_1 \wedge \cdots \wedge \varphi_m \wedge A_1(\overline{x_1}) \wedge \cdots
%  \wedge A_n(\overline{x_n}) \ \to \ A(\overline{x}), \tag{*}
%\end{equation*}
%where (a) $m \geq 0$ and $n \geq 0$; (b) $\varphi_i$ is an extraction
%formula; (c) $A_j \in \Gamma$ is a predicate of arity $k$; (d) $\overline{x_j} \in \VV^k$ where the variables in $\overline{x_j}$ are not
%necessarily mentioned in $\varphi_1, \ldots, \varphi_m$; (e) $A \in
%\Gamma$ is of arity $l$, and $\overline{x} \in \VV^l$ with all variables in  $\overline{x}$ occurring in the body of the rule. Moreover, an
%\emph{extraction program} $\Pi$ is a finite set of general extraction rules\footnote{Note that in \cite{AMRV16} only unary programs are considered since the focus of that work is annotating a single span inside a document. Here we are interested in extracting information using mappings, therefore we need to consider programs which themselves define mappings.}. A rule of the form \eqref{eq-ann-prog} is interpreted as defining a mapping stored into $A$, while using the information from extraction expressions $\varphi_1$ through $\varphi_m$, and mappings previously stored into the predicates $A_1$ though $A_n$. As in datalog \cite{AHV95}, we assume that each program has a unique output predicate. An extraction program $\Pi$ is {\em non-recursive} if it can be ordered in such a way that the head of a rule does not appear in the body of any previous rule in this ordering. An extraction program $\Pi$ is {\em tree-like}, if every rule in $\Pi$ is tree-like.
%
%Semantics of extraction programs is defined via ground predicates.
%A ground predicate over a document $d$ is an expression of the form $A(p_1,\ldots ,p_k)$,
%where $A \in \Gamma$ is of arity $k$ and $p_1,\ldots ,p_k \in \sub(d)$. Assume that  $\Lambda$ is a set of
%ground predicates over $d$. Then $\Lambda$ is said to satisfy the rule
%\eqref{eq-ann-rule} if for every variable assignment $\mu$ over $d$ such
%that $\mu \in \semd{\varphi_i}$ for every $i \in \{1, \ldots, m\}$, it holds
%that:
%\begin{center}
%  if $A_i(\mu(\overline{x_i})) \in \Lambda$ for all $i \in \{1,\ldots,n\}$, then also
%  $A(\mu(\overline{x})) \in \Lambda$,
%\end{center}
%where $\mu(\overline{x})$ is defined as a mapping assigning values to variables in $\overline{x}$ according to $\mu$.
%Moreover, $\Lambda$ is said to satisfy an extraction program $\Pi$ if $\Lambda$
%satisfies each rule in $\Pi$.
%
%To define the evaluation of an extraction program  over a document, we need to
%consider all sets of ground predicates over the document that satisfy the
%program. More specifically, given a document $d$, an extraction program $\Pi$
%over $d$ (with the output predicate $A$) and a ground predicate $A(p_1,\ldots ,p_k)$ over  $d$, we will consider $A(p_1,\ldots ,p_k)$ as a
%result of evaluating $\Pi$ over $d$ if we are certain about this mapping in
%the sense that $A(p_1,\ldots ,p_k)$  occurs in every  set of ground predicates  over $d$
%that satisfies $\Pi$. Formally, the evaluation of $\Pi$ over $d$, denoted  by
%$\textsc{Eval}(\Pi,d)$, is defined as follows (with $A$ being the output predicate of $\Pi$):
%\begin{multline*}
%  \{ A(p_1,\ldots ,p_k) \mid \text{for every set } \Lambda 
%      \text{ of ground predicates}\\ \text{ over } d
%  \text{ such that } \Lambda \text{ satisfies } \Pi,\\ \text{ it holds that }
%      A(p_1,\ldots ,p_k) \in \Lambda \}.
%\end{multline*}
%
%So how do extraction programs compare to \RGX-based extraction in terms of expressive power? Of course, if we only consider plain \RGX\ formulas and do not allow combining them, we know that extraction programs can define many more properties since they allow e.g. recursion. To make the comparison more fair, we will allow combining \RGX\ using algebraic operations of union, natural join and selection; that is, we will consider spanner algebras\footnote{Here we do not consider the string selection operator from \cite{FKRV15}, nor the content operator from \cite{AMRV16}, since these are not ``pure" extraction operations, and were shown in \cite{AMRV16} to cause a complexity-blowup. However, we do plan to see how the two operations relate in future work.} introduced in \cite{FKRV15}.
%
%It was shown in \cite{FKRV15} that \RGX\ formulas are equivalent to \VAStk\ automata, and that the algebra based on \VAStk\ automata is equivalent to \VASet\ automata. So what is the relation between the expressiveness of \VASet\ automata and extraction programs? As we next show, extraction programs subsume \VASet\ automata. In fact, one can even consider non-recursive extraction programs using only tree-like rules to obtain this result.
%
%\begin{proposition}
%  For every \VASet\ automaton there is an equivalent tree-like non-recursive
%  extraction program.
%\end{proposition}
%
%The proof here is based on the fact that unions of tree-like rules are equivalent to \RGX\ (Theorem \ref{lemma:utlstar-rgx}), thus allowing to define \RGX\ by programs. Furthermore, it is easy to see that programs are closed under union, join and selection, so the equivalences $\RGX\equiv\VAStk$ and $\VAStkUPJ \equiv \VASet$ give us the desired result. Whether non-recursive tree-like programs are in fact equivalent to \VASet\ automata remains an open problem, which we plan to address in future work.
%
%%%% Local Variables:
%%%% mode: latex
%%%% TeX-master: "main"
%%%% End:

\end{comment}


==> Expressiveness-of-RGX___new.tex <==
% Comparison of Span Regular Expressions vs Regex Formulas.

\section{Expressiveness of IE languages}\label{sec:expr}

In Section \ref{sec-unifying} we saw a unifying framework subsuming previous approaches to information extraction. As shown there, \RGX\ formulas of \cite{FKRV15} strictly subsume \SRGX\ of \cite{AMRV16}. However, the approach of \cite{AMRV16} also allows combining \SRGX\ formulas into rules. Therefore, in this section we study the exact connection between the two formalisms. We start by defining  rules based on \SRGX, and then isolate a simple subclass of such rules that is equivalent to \RGX. We also study how rules can be simplified by removing cycles, and  compare \RGX\ to more general classes of rules.

%, starting from simple rules based on span regular expressions.
%\SRGX, and moving up to the comparison of datalog-like rule language for \SRGX, and its relation with \RGX\ algebras, and different automata models for the two languages.

\subsection{Rules for information extraction}
Regex formulas allow the user to specify the shape of the span captured by 
some variable using an expression of the form $x\{\gamma\}$. For example, 
if we want to say that the string corresponding to the span captured by the 
variable $x$ belongs to the regular language $R$, we would write $x\{R\}$.
As we have seen in the previous section, this immediately makes \RGX\ 
formulas more expressive than \SRGX\ formulas, since the latter cannot constrain 
the shape of the span captured by a variable. So how can one specify that a
span captured by a variable inside a \SRGX\ formula has a specific shape? 

A natural
approach to solve this issue allows joining \SRGX\ formulas using 
a rule-like syntax \cite{AMRV16}. For instance, to specify that the content of the spans captured by 
the variable $x$ belongs to a language in the intersection of two regular expressions $R_1$ and $R_2$,
we can now write  $x.R_1  \wedge x.R_2$. Of course, since regular languages 
are closed under intersection, it is also possible to express this property using
\RGX, however, the resulting expression will generally be less intuitive 
than the simple rule above. One can see that the two approaches to information
extraction have slightly different design philosophies: on the one hand, we have 
the concise syntax of \RGX, and on the other hand we have a more visual approach
which combines \SRGX\ formulas into rules. In this section we explore how these two
approaches compare in terms of expressive power.

\smallskip

To do this, we first need to define a rule-based language for extracting
information from documents that is based on \SRGX\ formulas. In our language, 
we will allow two types of formulas: $R$ and $x.R$, where
$R$ is a \SRGX\ formula and $x$ a variable. The former is meant to be evaluated over the entire document,
while the latter applies to the span captured by the variable $x$. The semantics of the
extraction formula $R$  over a document $d$ is defined as above, and for $x.R$ as follows:
\begin{gather*}
  \semd{x.R} \ = \ \{ \mu \mid \exists s. (s,\mu)\in \sempd{x\{R\}} \}.
\end{gather*}

We can now define rules for extracting information from a document as conjunctions
of extraction formulas. Formally,
 an \emph{extraction rule} is an expression of the form:
\begin{equation*} \label{eq-ann-rule}
  \varphi = \varphi_0 \wedge x_1.\varphi_1 \wedge \cdots \wedge x_m.\varphi_m \tag{\dag}
\end{equation*}
where $m \geq 0$, all $\varphi_i$ are \SRGX\ formulas, and $x_i$ are variables\footnote{For simplicity we assume that there is only one formula applying to the entire document; namely $\varphi_0$. It is straightforward to extend the definitions below to include multiple formulas of this form.}. And while \cite{AMRV16} has a simple definition of the semantics of extraction rules, lifting this definition to the domain of (partial) mappings requires us to account for nondeterminism of our expressions. 
What we mean by this is perhaps best captured by a rule which is of the form $x+y \wedge x.ab^* \wedge y.ba^*$, where we first chose which variable is going to be mapped to the entire document, and then we need to satisfy its respective constraint. For instance, if $x$ is matched to the document, we want it to conform to the regular expression $ab^*$; however, in this case we do not really care about the content of $y$, so we should leave our mapping undefined on this variable. 

%The second challenge, ``ghost variables", refer to variables which are not linked to a specific part of a document, but can be assigned arbitrary spans. For instance, in a rule $\Sigma^* \wedge x.ab^*$, the variable $x$ does not really give us any information about the document itself, since it talks about arbitrary spans. What we really want is to link it to the rule applying to the entire document somehow; be it so that it appears in this formula itself (e.g. in $\Sigma^*x\Sigma^* \wedge x.ab^*$), or can reach it through other variables (e.g. in $\Sigma^*y\Sigma^* \wedge y.x \wedge x.ab^*$). We account for such behaviour as follows.

Formally, we will define when a rule of the form (\ref{eq-ann-rule}) is satisfied by a tuple of mappings $\overline{\mu}=(\mu_0,\mu_1,\ldots ,\mu_m)$. To avoid the problem mentioned above, we need the concept of {\em instantiated variables} in our tuple of mappings. For a rule $\varphi= \varphi_0 \wedge x_1.\varphi_1 \wedge \cdots \wedge x_m.\varphi_m$ and a tuple of mappings $\overline{\mu}=(\mu_0,\mu_1,\ldots ,\mu_m)$ we define the set of instantiated variables, denoted by $\ivar(\varphi,\overline{\mu})$ as the {\em minimal set} such that:
\begin{itemize}\itemsep=0pt
\item[-] $dom(\mu_0)\subseteq \ivar(\varphi,\overline{\mu})$; and
\item[-] If $x_i\in \ivar(\varphi,\overline{\mu})$, then $dom(\mu_i)\subseteq \ivar(\varphi,\overline{\mu})$.
\end{itemize}
Intuitively, we want to capture only the variables which are used in nondeterministic choices made by our rule. For instance, in case of the rule 
$x+y \wedge x.ab^* \wedge y.ba^*$, if we decide that $x$ should be matched to our document, then we will not assign a value to the variable $y$ and vice versa. We now define that a tuple of variables $\overline{\mu}=(\mu_0,\mu_1,\ldots ,\mu_m)$ satisfies $\varphi$ over a document $d$, denoted by $\overline{\mu}\models_d \varphi$, if the following holds:
\begin{itemize}\itemsep=0pt
\item[-] $\mu_0\in \semd{\varphi_0}$;
\item[-] If $x_i\in \ivar(\varphi,\overline{\mu})$ then $\mu_i \in \semd{x_i.\varphi_i}$;
\item[-] If $x_i\notin \ivar(\varphi,\overline{\mu})$ then $\mu_i = \emptyset$; and
\item[-] $\mu_i\sim \mu_j$ for all $i,j$.
\end{itemize}
Here the last condition will allow us to ``join'' all the mappings capturing each subformula $\varphi_i$ into one. The problem with nondeterminism is handled by the two rules in the middle, since we force all instantiated variables to take a value, and the non-instantiated ones to be undefined. Finally, the definition starts from our main subformula ($\varphi_0$) which refers to the entire document and serves as a sort of a root for our mappings.


We can now define the semantics of an extraction rule $\varphi$ over a document
$d$ as follows:
\begin{gather*}
  \semd{\varphi} \ = \ \{ \mu \mid \exists \overline{\mu} \text{ such that } \overline{\mu}\models_d \varphi \text{ and } \mu = \bigcup_i \mu_i \},
\end{gather*}
where $\bigcup_i \mu_i$ signifies the mapping defined as the union of all $\mu_i$.

Extraction rules allow us to define complex conditions about the
spans we wish to extract. For instance, if we wanted to extract all spans whose content
is a word belonging to (ordinary) regular expressions $R_1$ and $R_2$ at the same time, 
we could the rule $\Sigma^*\cdot x \cdot \Sigma^* \wedge x.R_1 \wedge x.R_2.$
More importantly, using extraction rules, we can now define valuations which can not be
defined using \RGX, since it can define mappings which are not hierarchical.
For instance, the rule $x\wedge x.ayaa \wedge x.aaza$ is one such rule, since it makes $y$ and $z$ overlap.
%To see this, consider a rule of the form $x \wedge x.a\cdot y \wedge x.a\cdot z$,
%which defines valuations where both $y$ and $z$ are part of the document after the initial letter $a$.
%Clearly, such a rule can not be defined using \RGX, since the spans assigned to $y$ and $z$ always have
%to be the same. 
In some sense, the ability of rules to use conjunctions of variables makes them
more powerful than \RGX\ formulas.% in some cases. 
On the other hand, the ability of \RGX\ formulas to use
disjunction of variables poses the same type of problems for \SRGX. 
Here one separating example would be the \RGX\ $\Sigma^{*} \cdot (x\{y\{\Sigma^{*}\}\cdot a\} \vee
    y\{x\{\Sigma^{*}\}\cdot a\}) \cdot \Sigma^{*}$. 
Therefore, we have the following:

\begin{proposition} \label{prop-rgx-rules}
Extraction rules and \RGX\ formulas are incomparable in terms of the expressive power.
\end{proposition}

Of course, a natural question now is which fragments of the two languages are equivalent.
%We address this question next.

\subsection{Unions of rules}

%%Of course, a natural question now is which fragments of the two languages are equivalent.
%In order to cover all \RGX\ formulas, we will show how unions of rules can be used to simulate the disjunction
%of variables. However, for this we also need to prune the class of rules we allow,
%since already a single rule can express properties beyond the reach of \RGX. As we have seen, 
%allowing conjunction of the same variable is problematic for \RGX. This leads us to the class
%of simple rules. An extraction rule is {\em simple}, if (1) it uses an expression formula {\it not} of 
%the form $x.R$ at most once; and (2) every variable appears at most once in an expression of the form
%$x.R$. However, even simple rules can go beyond \RGX.
%
%\begin{lemma}
%There is a simple extraction rule with no equivalent \RGX\ formula.
%\end{lemma}
%
%The result here is due to the fact that simple rules still allow ``cyclic" definitions such as $x.y \wedge y.ax$,
%which can make them un-satisfiable: a property which they do not share with \RGX. 
%%
%%MOVE TO DAG-LIKE 
%%
%%\bigskip
%%
%%HERE COMES THE TREE-LIKE STUFF
%%
%%
%A way around this is to prohibit
%such behaviour by forcing the rules to have a tree-like structure. In fact, this class of extraction
%rules was already considered in \cite{AMRV16}, as it allows faster evaluation than the class of all rules.
%In order to define the class of {\em tree-like rules}, we need to explain how each rule can be viewed as a graph.

%Of course, a natural question now is which fragments of the two languages are equivalent.

In order to cover all \RGX\ formulas, we will show how unions of rules can be used to simulate the disjunction
of variables. However, for this we also need to prune the class of rules we allow,
since already a single rule can express properties beyond the reach of \RGX. As we have seen, 
allowing conjunctions of the same variable is problematic for \RGX. Another thing that makes rules ``look different"
than \RGX\ is their ability to enforce cyclic behaviour through expressions of the form $x.y \wedge y.ax$.

A natural way to circumvent both of these shortcomings is to force the rules to have a tree-like structure. 
In fact, this class of extraction
rules was already considered in \cite{AMRV16}, as it allows faster evaluation than general rules.
In order to define the class of {\em tree-like rules}, we need to explain how each rule can be viewed as a graph.

To each extraction rule $\varphi=\varphi_0 \wedge x_1.\varphi_1 \wedge \cdots \wedge x_m.\varphi_m$ we associate a graph $G_\varphi$ defined as follows. The set of nodes of $G_{\varphi}$ contains all the variables $x_1,\ldots ,x_m$ plus one special node labelled $\texttt{doc}$ corresponding
to the formula $\varphi_0$.
There exists an edge $(x, y)$ between two variables in $G_{\varphi}$ if and only if there is an
\emph{extraction formula} $x.R$ in $\varphi$ such that $y$ occurs in
$R$. Furthermore, if the variable $x$ occurs in the formula $\varphi_0$, we add an edge $(doc,x)$ to $G_\varphi$.
Then we say that $\varphi$ is \emph{tree-like} if (1) every variable $x$ appears at most once on the left hand side of an expression of the form
$x.R$; and (2) $G_{\varphi}$ is a tree rooted at $\texttt{doc}$. We can now show that the class of tree-like rules is indeed subsumed by \RGX.
%Then we say that $\varphi$ is \emph{tree-like} if (1) it uses an expression {\it not} of 
%the form $x.R$ at most once; (2) every variable $x$ appears at most once on the left hand side of an expression of the form
%$x.R$; and (3) $G_{\varphi}$ is a rooted-forest (i.e.\ a set of
%rooted-trees). We can now show that the class of tree-like rules is indeed subsumed by \RGX.

\begin{lemma}\label{lemma:tl-rgx}
  Every \emph{tree-like} rule can be transformed into an equivalent
  \(\RGX\).
\end{lemma}

As we know, \RGX\ alone are more expressive than any single rule, but by allowing unions of 
tree-like rules, we get a class of extraction rules capturing \RGX\ formulas. Formally,
{\em union of tree-like rules} is a set of tree-like rules $A$. The semantics over a 
document $d$ is defined as 
\begin{gather*}
  \semd{A} \ = \ \{ \mu \mid \mu \text{ is a variable assignment over }
      d\\
   \hspace{65pt} \text{ such that } \mu \in \semd{\varphi}, \text{ for some } \varphi\in A \}.
\end{gather*}
With this in hand, we can now better understand the connection between rules and \RGX:

\begin{theorem}\label{lemma:utlstar-rgx}
Unions of tree-like rules are equivalent to \(\RGX\) formulas.
\end{theorem}

The proof of this theorem relies on the fact that \RGX\ formulas are equivalent to unions of functional \RGX\ which do not use disjunctions of (expressions containing) variables. The latter can be then easily expressed using a tree-like rule, giving us one direction of the theorem. The other direction follows from Lemma \ref{lemma:tl-rgx} and the fact that \RGX\ formulas are closed under disjunction. Analysing the proof also shows us that the transformation is exponential in both directions.

%The proof of this theorem relies on the fact that \RGX\ formulas are equivalent to 
%variable stack (\VAStk) automata \cite{FKRV15}. Furthermore, \cite{FKRV15} also shows that every
%\VAStk\ automaton can be transformed into a \VAStk\ automaton which consists of disjoint paths
%connecting the starting and the accepting state, also known as path-union automaton, or \PUStk.
%Using this, we can show that every \RGX\ is equivalent to a disjunction of \RGX\ formulas which
%do not use disjunction of (expressions containing) variables, since each such expression can
%be viewed as one path in \PUStk\ automaton. Finally, we show that each \RGX\ not containing
%disjunctions of variables can be defined using a tree-like rule, therefore allowing us to express
%an arbitrary \RGX\ as a union of tree-like rules. The other direction of the theorem follows from 
%Lemma \ref{lemma:tl-rgx} and the fact that \RGX\ formulas are closed under disjunction.


%\smallskip

%Apart from knowing that the classes of \RGX\ formulas and unions of tree-like rules are equivalent, one might also be
%interested in how difficult it is to compute the equivalent expression. Here we can show that to define
%a single tree-like rule one requires an exponential size \RGX\ formula,
%since extraction rule can contain \SRGX\ which repeat the same variable multiple times. 
%On the other hand, defining a \RGX\ by union of tree-like rules requires an exponential number of rules, because to represent
%a \RGX\ using \PUStk\ we might already need exponentially many paths in our automaton.

\subsection{Eliminating cycles from rules}

%WILL INTEGRATE THIS INTO SEC 3.2. AFTERWARDS IF CRISTIAN MAKES ME
%
%The result here is due to the fact that simple rules still allow ``cyclic" definitions such as $x.y \wedge y.ax$,
%which can make them un-satisfiable: a property which they do not share with \RGX. So how can we restrict the class
%of rules in order to prohibit such behaviour? For this, we first need to consider the graph structure of each rule.
%
%To each extraction rule $\varphi$ we associate a graph $G_\varphi$ defined as follows. The
%set of nodes of $G_{\varphi}$ is the set of variables occurring in $\varphi$, and
%there exists an edge $(x, y)$ in $G_{\varphi}$ if and only if there is an
%\emph{extraction formula} $x.R$ in $\varphi$ such that $y$ occurs inside 
%$R$. If the graph $G_\varphi$ contains no cycles, we call the rule $\varphi$ a {\em dag-like} rule,
%since it resembles a directed acyclic graph. It is then not difficult to see that each dag-like
%rule has an equivalent \RGX.
%
%\begin{lemma}\label{lemma:dag-rgx}
%  Every \emph{dag-like} rule can be transformed into an equivalent \(\RGX\).
%\end{lemma} 
%
%What is perhaps more surprising, is the fact that we can rewrite each simple rule into an equivalent dag-like rule; that is,
%we can remove cycles from our rules.


%EMPH ON SAT:
%The example showing that not all simple rules can be expressed as \RGX\ relies on the fact that rules can define cycles in their associated graph and can as such force them to not be satisfiable. This is easily circumvented by going to tree-like rules, but this jump seems rather ad hoc, since it does not answer the question of what happens with simple rules that are satisfiable? What we show in this subsection is that if a simple rule is satisfiable we can remove cycles from it, and that we can then transform it to a union of tree-like rules.

%RULES ONLY, NOT MENTIONING SAT:


%The example showing that not all simple rules can be expressed as \RGX\ relies on the fact that rules can define cycles in their associated graph. This is easily circumvented by going to tree-like rules, but the jump seems rather ad hoc, since there is a more general class of rules which prohibit such behaviour; namely dag-like rules. We call a rule $\varphi$ a {\em dag-like rule}, if the graph $G_\varphi$ contains no cycles. Perhaps surprisingly, one can actually show that each simple rule can be rewritten into a dag-like rule in polynomial time by eliminating the cycles from it. In this subsection we present an algorithm for cycle elimination from rules, and discuss how simple rules are connected to tree-like rules and \RGX.

In the previous subsection we isolated a class of rules whose unions are equivalent to \RGX\ formulas. To do this, we prohibited the rules to use the conjunction of the same variable twice, and forced them to have a tree-like structure. And while prohibiting arbitrary conjunction was shown to be crucial, we have still not answered if the capability of rules to define cycles is really an obstacle, or if they can be removed. Consider for instance a rule of the form  $x \wedge x.y \wedge y.x$, whose underlying graph is cyclic. This rule is clearly equivalent to $x\wedge x.y$, that requires no cycles in order to express the same property. In this section we consider the question whether cycles can be eliminated from rules, and somewhat surprisingly show that, while generally not possible, in the case when all expressions defining a rule are functional span \RGX\ formulas this is indeed true. %We also discuss how this relates to the difference in expressiveness of different classes of rules.

%as cyclic rules could still be equivalent to \RGX\ formulas in terms of mappings they define. For instance, the rule $x \wedge x.y \wedge y.xz$ is easily seen to be equivalent to the \RGX\ $x\{y\{z\{\varepsilon\}\}\}$. Surprisingly, in this section we show that unions cyclic rule which prohibit arbitrary conjunctions are indeed equivalent to \RGX. We start by showing something even more surprising; namely, that one can eliminate cycles from cyclic rules without losing expressive power. We then show how such acyclic rules are connected to tree-like rules and \RGX. 

Let us formally define the classes of rules we will consider in this section. First, as discussed above, the capability of an extraction rule to use conjunctions of the same variable multiple times already takes them outside of the reach of \RGX. Therefore the most general class of rules we will consider disallows that type of behaviour. We call such rules {\em simple rules}. Formally, an extraction rule $\varphi = \varphi_0 \wedge x_1.\varphi_1 \wedge \cdots \wedge x_m.\varphi_m$ is {\em simple}, if all $x_i$ are pairwise distinct. Note that simple rules can still be ``cyclic" in nature, namely, the graph $G_\varphi$ associated with the rule $\varphi$ can have cycles. We call a rule $\varphi$ {\em dag-like}, if the graph $G_\varphi$ contains no cycles. Furthermore, a rule $\varphi$ is called {\em functional}, if all of the \SRGX\ formulas $\varphi_0, \ldots ,\varphi_m$ are functional \RGX\ formulas.

To answer the question whether cycles can be eliminated from rules, let us consider the most general case; namely, simple rules. It is straightforward to see that in a rule of the form $x+y \wedge x.(y+\Sigma^*) \wedge y.(x+\Sigma^*)$, the cycle formed by $x$ and $y$ can not be broken and the rule can not be rewritten as a single dag-like rule. The main obstacle here is the fact that in each part of the rule we make a nondeterministic choice which can then affect the value of all the variables.

However, there is one important class of expressions, which would prohibit our rules to define properties such as the one above; that is, functional span regular expressions. The notion of functionality, first introduced in \cite{FKRV15}, was shown to be crucial for having a well-behaved fragment of \RGX\ formulas, and it also has a profound effect on complexity of formula evaluation, since it brings it down from $\NP$-hard to tractable (see Section \ref{sec:eval}). As defined previously, functional formulas force that the variables used on the two sides of a disjunction are always the same, and furthermore, require concatenated expressions to share no variables (thus also forcing the star operator to be allowed only over variable free formulas). Somewhat surprisingly, we can show that in the case of functional rules cycles can always be removed, and in fact, converting a simple rule that is functional into a dag-like rule takes only polynomial time. 

%Take therefore an arbitrary simple rule that is {\em functional}.
%We start by analysing what sort of a value can a mapping assign to the variables which form a cycle.
%For this take any rule $\varphi$ and assume that there is a simple cycle $x_1,\ldots ,x_n$ appearing in $G_\varphi$ and a mapping $\mu$ satisfying $\varphi$. Then the following must hold:
%\begin{enumerate}
%\item {\em All variables in the cycle must be assigned the same value.} This follows from the fact that in a simple rule each edge $(x,y)$ in $G_\varphi$ implies that $\mu(x)$ contains $\mu(y)$.
%\item {\em Every variable reachable from a cycle, but not inside it, must be assigned the empty content.} This follows from the observation above, plus the fact that edges $(x,y)$ and $(x,y)$ in $G_\varphi$ imply that $\mu(y)$ and $\mu(z)$ are disjoint.
%\item {\em If the cycle has a chord, then all the variables inside it must be assigned the empty content.} Here a chord means that we have a path from some $x_i$ to some $x_j$ inside $G_\varphi$ which consists of nodes not belonging to our cycle,  or there is a direct edge between them which is not part of the cycle. In the case there is an intermediate node, we know that it must be assigned $\varepsilon$, therefore $x_j$ and all other nodes in the cycle must be $\varepsilon$ as well. If the edge is direct, then by the definition of a chord, $x_j$ is not a successor of $x_i$ in the cycle, so just as in the previous case, the content of the successor of $x_i$ and the content of $x_j$ must be disjoint and equal, which is only possible if they are $\varepsilon$.
%\end{enumerate}
%
%The procedure for eliminating cycles from simple rules is based on the following colouring scheme for a graph
%$G_{\varphi}$ associated with the rule $\varphi$. Let $\varphi$ be an extraction rule with variables $x_1,\ldots x_n$. We will
%colour a node $x_i$ {\em black} if:
%\begin{itemize}
%\item $x_i.\varphi_i$ appears in $\varphi$ and $\varphi_i$ has at least one symbol of the alphabet which is not under the star operator $*$; that is, the variable $x_i$ must contain at least one occurrence of an alphabet letter.
%\end{itemize}
%We then paint the graph by assigning the colour {\em red} to all black nodes, and all nodes which can reach a black node. All other nodes are coloured {\em green}. It is clear that this procedure can be carried out in polynomial time, since reachability takes only polynomial time. Note that in a black node coming from a conjunct of the form $x_i.\varphi_i$, the content of each variable appearing in $\varphi_i$ must be {\em strictly} contained in the content of the variable $x_i$, because $\varphi_i$ is functional. Also note that each cycle has to be coloured using the same color.
%
%If we now have a simple cycle $x_1,\ldots ,x_n$ we can eliminate it by considering its color:
%\begin{itemize}
%\item {\em If the cycle is coloured red, then the rule is not satisfiable, so we can replace it by an arbitrary unsatisfiable dag-like rule.} We have two cases here. First, if a rule contains a black node, then the content of its successor must be strictly contained inside its own content, which can not happen by the analysis above. Second, if a node $x$ in the cycle can reach some black node not inside the cycle, then its content must be different from $\varepsilon$ (because the content of the black node is different from it), but then $x$ must also strictly contain the content of its successor in the cycle, which is a contradiction by the above analysis.
%\item {\em If the cycle is green we can simplify it using an auxiliary variable.} Let $u_1, \ldots, u_m$ be the variables that are not
%  part of the cycle and for which there is an edge $(u_i, x_1)$. Let $y_1,
%  \ldots, y_l$ be the variables that are not part of the cycle and are reachable
%  from some $x_i$ (they must have empty content, as proved before). We then add an auxiliary variable $w$ and and edge from it to $x_1$. Each expression associated with some $u_i$ is changed so that it uses $w$ instead of $x_1$, and all expression associated with some $y_i$ are changed to $y_i.\varepsilon$. Next, an expression $x_i.\varphi_i$ is changed to  $x_i.\varphi_i'$, where $\varphi_i'$ maintains the ordering of variables in $\varphi_i$ that are not under a star operator and removes all other letters or starred subexpressions, for $i<n$. For $x_n$, we replace the occurrence of $x_1$ by $\Sigma^*$. This yields an equivalent \emph{simple} rule without the mentioned cycle.
%\end{itemize}
%
%As an example of how the rewriting above works, consider the rule $x.y \wedge y.z \wedge z.ux.$
%This rule can be rewritten to $w.x \wedge x.y \wedge y.z \wedge z.u \wedge u.\varepsilon$.
%
%\domagoj{We should say where is the functionality of rules used!}
%
%Of course, here we explained only how a single cycle can be removed, but how do we transform a rule with multiple cycles in its graph? For this we start by identifying the strongly connected components of our graph $G_\varphi$. Each component can then be either: (a) a single node, (b) a simple cycle, or (c) a simple cycle with additional edges. In the latter two cases, if any component is coloured red, we know that the rule is unsatisfiable, so we can replace it by an arbitrary unsatisfiable dag-like rule. In the case they are coloured green, we can deploy the procedure above to remove the cycles, taking care that in the case (b) our variables can take an arbitrary, but always equal value, while in the case (c) they must be equal to the empty content. In both cases, all the variables reachable from the component are made $\varepsilon$. Since strongly connected components can be computed in polynomial time, we obtain the following.

\begin{theorem}\label{thm:simple_to_dag}
For every simple rule that is functional there is an equivalent (functional) dag-like rule. Moreover, we can obtain the equivalent rule in polynomial time.
\end{theorem}

We now know that cycles can be eliminated from functional rules, but is there any way to simplify rules that are not functional? As it turns out, although functional and non-functional rules are not equivalent, every non-functional simple rule can in fact be expressed as a union of functional rules. 

\begin{proposition}\label{prop:nonfunc}
Every non-functional simple rule is equivalent to a union of functional simple rules.
\end{proposition}

To see this, observe first that every non-functional \SRGX\ formula can be expressed as a (potentially exponentially big) union of functional \SRGX\ formulas (Theorem \ref{th-stack_rgx}). Therefore, each non-functional rule $\varphi_0 \wedge x_1.\varphi_1 \wedge \cdots \wedge x_m.\varphi_m$ can be rewritten into a rule whose formulas $\varphi_i$ are unions of functional \SRGX. Now each such rule can be transformed into a union of functional rules by taking all the possible disjunctions (of which there will generally be exponentially many). 



\subsection{Regex vs. rules}

One final thing we would like to determine is the connection of the more general classes of simple and dag-like rules to \RGX. We will start by considering functional rules and comparing them to functional \RGX\ formulas. As shown in Theorem \ref{lemma:utlstar-rgx}, unions of tree-like rules are equivalent to \RGX. It is straightforward to see that this is still true when we consider functional rules and \RGX. Therefore to connect functional rules which are not necessarily tree-like to \RGX, we will show how and when can they be viewed as tree-like.

First, observe that a functional \RGX\ formula is always satisfiable; namely, there is always a document on which there is an assignment satisfying this formula. Similarly, every functional tree-like rule is also satisfiable. On the other hand, a functional simple rule $x\wedge x.y \wedge y.ax$ is clearly not satisfiable, since it forces $x$ and $y$ to be equal and different at the same time. Therefore, to link functional rules with \RGX, we need to consider only the satisfiable ones. As we know that each functional simple rule has an equivalent dag-like rule, we start there.


\begin{theorem}\label{thm:dag_to_tree}
Every functional dag-like rule that is satisfiable  is equivalent to a union of functional tree-like rules.
\end{theorem}

The idea of the proof here is similar to the cycle elimination procedure of Theorem \ref{thm:simple_to_dag}, but this time considering undirected cycles. One can show that eliminating undirected cycles results in a double exponential number of tree-like rules. In case that the rule was not satisfiable, our algorithm will simply abort.

%The idea of the proof here is similar to the cycle elimination procedure above, but this time we need to consider undirected cycles, or more precisely, we consider all pairs of nodes which are linked by two or more distinct paths. Such undirected cycles are then removed based on whether the final node is coloured green or red. Furthermore, one can show that eliminating undirected cycles results in a double exponential number of tree-like rules. In case that the rule was not satisfiable, our algorithm will simply abort.

With this at hand, we can now also describe the relationship between functional simple rules and \RGX.

\begin{theorem}\label{thm:simple_to_rgx}
The class of functional \RGX\ formulas is equivalent to unions of satisfiable functional simple rules.
\end{theorem}

As we have shown, simple rules are equivalent to dag-like rules in the functional case. It is not difficult to see that each functional dag-like rule has an equivalent functional \RGX. On the other hand, we have also shown that each satisfiable functional dag-like rule can be expressed as a union of functional tree-like rules. And while a single dag-like rule is not enough to express an arbitrary \RGX\, similarly as in the case of tree-like rules, we can show that their unions can.

%Whether the same holds in the case of non functional rules is not entirely clear, as general \RGX\ formulas can be unsatisfiable. We conjecture that in this case general \RGX\ formulas are equivalent in expressive power to unions of simple rules.

Since we know (see Theorem \ref{th-stack_rgx} and comments below) that each \RGX\ is equivalent to a union of functional \RGX\ formulas (with the union being empty when \RGX\ is not satisfiable), we can also get a more general result.

\begin{theorem}\label{thm:rgx:simple}
The class of \RGX\ formulas is equivalent to unions of functional simple rules.
\end{theorem}



%\subsection{Extraction programs}
%
%Using unions is only a small extension to extraction rules. To harness the full power of the language based on such rules, the authors in \cite{AMRV16} allow combining them using datalog-like programs. In this subsection we explore how such a language compares to automata models for \RGX\ formulas and their algebraic closures.
%
%In order to define datalog programs based on extraction rules, we first extend rules with the ability to use arbitrary arity predicates. For this, let $\Gamma$ be a finite alphabet of predicates (of not necessarily same arity), which is disjoint from the alphabet $\Sigma$ and the set of variables $\VV$. 
% A \emph{general extraction rule} is an expression of the form:
%\begin{equation*} \label{eq-ann-prog}
%  \varphi_1 \wedge \cdots \wedge \varphi_m \wedge A_1(\overline{x_1}) \wedge \cdots
%  \wedge A_n(\overline{x_n}) \ \to \ A(\overline{x}), \tag{*}
%\end{equation*}
%where (a) $m \geq 0$ and $n \geq 0$; (b) $\varphi_i$ is an extraction
%formula; (c) $A_j \in \Gamma$ is a predicate of arity $k$; (d) $\overline{x_j} \in \VV^k$ where the variables in $\overline{x_j}$ are not
%necessarily mentioned in $\varphi_1, \ldots, \varphi_m$; (e) $A \in
%\Gamma$ is of arity $l$, and $\overline{x} \in \VV^l$ with all variables in  $\overline{x}$ occurring in the body of the rule. Moreover, an
%\emph{extraction program} $\Pi$ is a finite set of general extraction rules\footnote{Note that in \cite{AMRV16} only unary programs are considered since the focus of that work is annotating a single span inside a document. Here we are interested in extracting information using mappings, therefore we need to consider programs which themselves define mappings.}. A rule of the form \eqref{eq-ann-prog} is interpreted as defining a mapping stored into $A$, while using the information from extraction expressions $\varphi_1$ through $\varphi_m$, and mappings previously stored into the predicates $A_1$ though $A_n$. As in datalog \cite{AHV95}, we assume that each program has a unique output predicate. An extraction program $\Pi$ is {\em non-recursive} if it can be ordered in such a way that the head of a rule does not appear in the body of any previous rule in this ordering. An extraction program $\Pi$ is {\em tree-like}, if every rule in $\Pi$ is tree-like.
%
%Semantics of extraction programs is defined via ground predicates.
%A ground predicate over a document $d$ is an expression of the form $A(p_1,\ldots ,p_k)$,
%where $A \in \Gamma$ is of arity $k$ and $p_1,\ldots ,p_k \in \sub(d)$. Assume that  $\Lambda$ is a set of
%ground predicates over $d$. Then $\Lambda$ is said to satisfy the rule
%\eqref{eq-ann-rule} if for every variable assignment $\mu$ over $d$ such
%that $\mu \in \semd{\varphi_i}$ for every $i \in \{1, \ldots, m\}$, it holds
%that:
%\begin{center}
%  if $A_i(\mu(\overline{x_i})) \in \Lambda$ for all $i \in \{1,\ldots,n\}$, then also
%  $A(\mu(\overline{x})) \in \Lambda$,
%\end{center}
%where $\mu(\overline{x})$ is defined as a mapping assigning values to variables in $\overline{x}$ according to $\mu$.
%Moreover, $\Lambda$ is said to satisfy an extraction program $\Pi$ if $\Lambda$
%satisfies each rule in $\Pi$.
%
%To define the evaluation of an extraction program  over a document, we need to
%consider all sets of ground predicates over the document that satisfy the
%program. More specifically, given a document $d$, an extraction program $\Pi$
%over $d$ (with the output predicate $A$) and a ground predicate $A(p_1,\ldots ,p_k)$ over  $d$, we will consider $A(p_1,\ldots ,p_k)$ as a
%result of evaluating $\Pi$ over $d$ if we are certain about this mapping in
%the sense that $A(p_1,\ldots ,p_k)$  occurs in every  set of ground predicates  over $d$
%that satisfies $\Pi$. Formally, the evaluation of $\Pi$ over $d$, denoted  by
%$\textsc{Eval}(\Pi,d)$, is defined as follows (with $A$ being the output predicate of $\Pi$):
%\begin{multline*}
%  \{ A(p_1,\ldots ,p_k) \mid \text{for every set } \Lambda 
%      \text{ of ground predicates}\\ \text{ over } d
%  \text{ such that } \Lambda \text{ satisfies } \Pi,\\ \text{ it holds that }
%      A(p_1,\ldots ,p_k) \in \Lambda \}.
%\end{multline*}
%
%So how do extraction programs compare to \RGX-based extraction in terms of expressive power? Of course, if we only consider plain \RGX\ formulas and do not allow combining them, we know that extraction programs can define many more properties since they allow e.g. recursion. To make the comparison more fair, we will allow combining \RGX\ using algebraic operations of union, natural join and selection; that is, we will consider spanner algebras\footnote{Here we do not consider the string selection operator from \cite{FKRV15}, nor the content operator from \cite{AMRV16}, since these are not ``pure" extraction operations, and were shown in \cite{AMRV16} to cause a complexity-blowup. However, we do plan to see how the two operations relate in future work.} introduced in \cite{FKRV15}.
%
%It was shown in \cite{FKRV15} that \RGX\ formulas are equivalent to \VAStk\ automata, and that the algebra based on \VAStk\ automata is equivalent to \VASet\ automata. So what is the relation between the expressiveness of \VASet\ automata and extraction programs? As we next show, extraction programs subsume \VASet\ automata. In fact, one can even consider non-recursive extraction programs using only tree-like rules to obtain this result.
%
%\begin{proposition}
%  For every \VASet\ automaton there is an equivalent tree-like non-recursive
%  extraction program.
%\end{proposition}
%
%The proof here is based on the fact that unions of tree-like rules are equivalent to \RGX\ (Theorem \ref{lemma:utlstar-rgx}), thus allowing to define \RGX\ by programs. Furthermore, it is easy to see that programs are closed under union, join and selection, so the equivalences $\RGX\equiv\VAStk$ and $\VAStkUPJ \equiv \VASet$ give us the desired result. Whether non-recursive tree-like programs are in fact equivalent to \VASet\ automata remains an open problem, which we plan to address in future work.
%
%%%% Local Variables:
%%%% mode: latex
%%%% TeX-master: "main"
%%%% End:


==> Extraction-Programs.tex <==
% Comparison of Annotation Programs vs Variable Automata.

\section{Expressiveness of Annotation Programs}

In this section, we will analyze and compare the expressiveness of
\emph{annotation programs} with that of the \emph{variable automata} defined
in~\cite{FKRV15}. For this, we distinguish a special kind of program,
\emph{non-recursive annotation programs}, that use no recursion in the
usual datalog sense.

\begin{proposition}
  For every vset-automaton there is an equivalent \emph{tree-like non-recursive
  annotation programs}.
\end{proposition}

\begin{proof}
  From~\cite{FKRV15}, we already know that $\VAStkUPJ \equiv \VASet$, and from
  Proposition~\ref{lemma:utlstar-rgx}, we know that $\RGX$ is equivalent to
  \emph{tree-like rule sets}. Therefore, it suffices to show that we may
  simulate the $\cup, \pi, \Join$ algebraic operators using non-recursive
  tree-like rules.

  To simulate \emph{union} ($\cup$) we may use \emph{rule sets}. To simulate
  \emph{projection} ($\pi$) we use may use rules of the form $A(x_1,\ldots,x_n)
  \rightarrow A_{\pi}(y_1,\ldots,y_m)$ where $\{y_1,\ldots,y_m\} \subseteq
  \{x_1,\ldots,x_n\}$. Finally, for \emph{joins} ($\Join$), we may use rules of
  the form $A(x_1,\ldots,x_n) \wedge B(y_1,\ldots,y_m) \rightarrow
  C(z_1,\ldots,z_l)$ where $\{z_1,\ldots,z_l\} = \{x_1,\ldots,x_n\} \cap
  \{y_1,\ldots,y_m\}$.
\end{proof}

Open problem:
\begin{proposition}
  \emph{Non-recursive annotation programs} and vset-automata are equivalent.
\end{proposition}

==> Introduction.tex <==
% Preliminary concepts and definitions.

\section{Introduction}
With the abundance of different formats arising in practice these days, there is a great need for methods extracting singular pieces of data from a variety of distinct files. This process, known as information extraction, or IE for short, is particularly prevalent in big corporations that manage systems of increasing complexity which need to incorporate data coming from different sources. As a result, a number of systems supporting the extraction of information from text-like data have appeared throughout the years \cite{KLRRVZ08,Cunningham02,SDNR07}, and the topic received a substantial coverage in research literature (see \cite{Kimelfeld14} for a good survey).

Historically, there have been two main approaches to information extraction: the {\em statistical} approach utilising machine-learning methods, and the {\em rule-based} approach utilising traditional finite-language methods. In this paper we focus on the rule-based approach to information extraction for two reasons. First, rule-based information extraction is founded on methods traditionally used by the database community (such as logic, automata, or datalog-based languages) and has therefore enjoyed a great amount of coverage in the database literature \cite{FKRV15,FKRV14,freydenberger2016document,AMRV16}. Second, as argued by \cite{Kimelfeld14,ChiticariuLR13}, due to their simplicity and ease of use, rule-based systems seem to be more prevalent in the industrial solutions.

Generally, most rule-based information extraction frameworks deploy some form of regular-like expressions as the core mechanism for extracting the data  \cite{CM99,FKRV15,AMRV16}. Perhaps the best representative of this approach are the regular expressions with capture variables introduced in \cite{FKRV15}, called {\em regex formulas}, which form the basis of IBM's commercial IE tool SystemT \cite{KLRRVZ08}. In this setting, documents being processed are viewed as strings, which is a natural assumption for a wide variety of formats in use today (e.g. plain text, CSV files, JSON documents, etc). The pieces of information we want to extract are captured by {\em spans}, which are simply intervals inside the string representing our document, namely, spans are defined by the starting and ending points of some substring. Regex formulas are now used to specify, through regular expressions and variables, the spans that will be extracted. 

%%SHORT VERSION (AND UGLY)
%Historically, there have been two main approaches to information extraction: the {\em statistical} approach utilizing machine-learning methods, and the {\em rule-based} approach utilizing traditional finite-language methods. In this paper we focus on rule-based IE, since this approach has a strong rooting in the database literature \cite{FKRV15,FKRV14,freydenberger2016document,AMRV16}. Generally, most rule-based information extraction frameworks deploy some form of regular-like expressions as the core mechanism for extracting the data  \cite{CM99,FKRV15,AMRV16}. Perhaps the best representative of this approach are the regular expressions with capture variables introduced in \cite{FKRV15}, called {\em regex formulas}, which form the basis of IBM's commercial IE tool SystemT \cite{KLRRVZ08}. In this setting documents being processed are viewed as strings, which is a natural assumption for a wide variety of formats in use today (e.g. plain text, CSV files, JSON documents, etc.). The pieces of information we want to extract are captured by {\em spans}, which are simply intervals inside the string representing our document (that is, spans are defined by the starting point and the ending point of some substring). Regex formulas are now used to parse these strings, with variables storing {\em spans}.


Once spans have been extracted using regular-like expressions, most IE frameworks allow combining them and controlling their structure through a variety of different methods. For instance, \cite{FKRV15} permits manipulating spans extracted by regex formulas using algebraic operations, while \cite{AMRV16} and \cite{SDNR07} deploy datalog-like programs to obtain a more general way of defining relations over spans. Unlike regex, which specify variable filters explicitly inside formulas, \cite{AMRV16} uses a more visual approach implemented through {\em extraction rules}. These permit constraining the shape of a span captured inside a variable separately.

The way that most frameworks view information extraction is by defining a relation over spans. For example, in regex formulas of \cite{FKRV15}, all variables must be assigned in order to produce an output tuple, and a similar thing happens with the rule-based language of \cite{AMRV16}. However, in practice we are often working with documents which have missing information or optional parts, and would therefore like to maximise the amount of information we extract. To illustrate this, consider a CSV file\footnote{CSV, or comma separated values, is a simple table-like format storing information separated by commas and new lines.} containing land registry records about buying and selling property. In Table \ref{tab-csv} we give a few rows of such a document, where $\spa$ represents space and $\eol$ the new line symbol. Some sellers in this file have an additional field which contains the amount of tax they paid when selling the property. If we are extracting information about sellers (for instance their names) from such a file, we would then like to also include the tax information when the latter is available. However, if we are set on extracting relations, this will not be possible, since all variables need to be assigned in order to produce an output. %, thus causing us to miss some of the desired data.

\begin{table}
\begin{center}
{
\def\arraystretch{1.2}
\renewcommand{\familydefault}{\ttdefault}\normalfont
\begin{tabular}{l}
Seller:$\spa$John,$\spa$ID75\eol\\
{Buyer:}$\spa$Marcelo,$\spa$ID832,$\spa$P78\eol\\
Seller:$\spa$Mark,$\spa$ID7,$\spa$\$35,000\eol \vspace{-5pt}\\
\hspace{55pt}$\vdots$
\end{tabular}
}
\end{center}
\vspace*{-10pt}
\caption{Part of a CSV document containing information about buying and selling property.}
\vspace*{-20pt}
\label{tab-csv}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%
%OLD:
%Apart from the inability to capture partial or incomplete information, some further shortcomings of previous approaches are that defining the semantics of extraction expressions cannot be done in a fully declarative way \cite{FKRV15}, or that they assign arbitrary spans to variables when these are not matched against the document \cite{AMRV16}. Furthermore, not much is known about how these approaches compare in terms of expressive power, and apart from some preliminary studies on their computational properties \cite{freydenberger2016document,AMRV16}, we do not have a good understanding of how difficult it is to evaluate these languages, nor of the complexity of their main static analysis tasks.

%In order to overcome these issues, we propose a general framework subsuming several previous approaches to IE. %, and allowing us to handle incomplete data.
%For this, we consider core extraction mechanisms such as variants of regular expressions and automata, and extend them in order to accommodate incompleteness. We start with regex formulas of \cite{FKRV15} as the base, and redefine their semantics in such a way that they output {\em mappings} in place of relations, as it was done for the SPARQL query language in the Semantic Web context \cite{PAG09}. This allows us to capture optional parts of documents, such as in the example from Table~\ref{tab-csv}, since our expression will output a mapping that binds an extra variable to the tax data only when the latter is present in the document (otherwise we only extract the name of the seller). Furthermore, the generality of mappings allows us to have a simple declarative semantics of regex formulas. We also extend the automata models of \cite{FKRV15} to this new setting and show when they capture the extraction expressions under the new semantics.
%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this paper, we propose a theoretical framework that extends both regex formulas~\cite{FKRV15} and extraction rules~\cite{AMRV16} in order to support incomplete information extraction. 
Specifically, we take regex formulas of \cite{FKRV15} as our core extraction mechanism, and  redefine their semantics in such a way that they output {\em mappings} in place of relations, as it was done for the SPARQL query language in the Semantic Web~\cite{PAG09}. This allows us to capture optional parts of documents, such as in the example from Table~\ref{tab-csv}, since our expression will output a mapping that binds an extra variable to the tax data only when the latter is present in the document. % (otherwise we only extract the name of the seller).
 Furthermore, the generality of mappings allows us to have a simple declarative semantics of regex formulas as opposed to parse trees of \cite{FKRV15}. We also extend the automata models of \cite{FKRV15} to this new setting and show when they capture the extraction expressions under the new semantics.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%
%OLD
%Next, we study how the formal IE frameworks introduced previously compare in terms of expressive power. Here we start with regex formulas of \cite{FKRV15} and span regular expressions of \cite{AMRV16}, since these form the information extraction base of the two frameworks. We prove that both languages are special cases of our definition\footnote{Note that in this paper we do not consider the content operator of \cite{AMRV16}, nor the string selection of \cite{FKRV15}, since these do not directly extract information, but rather compare two pieces of existing data.}, with the latter being less expressive. We then analyse extraction rules of \cite{AMRV16} showing how these can be used to capture regex formulas and also provide a method for simplifying such rules. 
%%Note that in our analysis we consider only core extraction mechanisms, such as variants of regular expressions and automata (we plan to examine algebras, and recursive datalog-based languages in the future). Furthermore, we do not consider the content operator of \cite{AMRV16}, nor the string selection of \cite{FKRV15}, since these do not directly extract information, but compare two pieces of existing data.
%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Since not much is known about how different IE frameworks compare in terms of expressive power, we next study this problem focusing on two previously introduced approaches: spanners \cite{FKRV15} and extraction rules \cite{AMRV16}. We start with regex formulas of \cite{FKRV15} and span regular expressions of \cite{AMRV16}, since these form the information extraction base of the two frameworks. We prove that both languages are special cases of our definition\footnote{Note that in this paper we do not consider the content operator of \cite{AMRV16}, nor the string selection of \cite{FKRV15}, since these do not directly extract information, but rather compare two pieces of existing data.}, with the latter being less expressive. We then analyse extraction rules of \cite{AMRV16} showing how these can be used to capture regex formulas and also provide a method for simplifying such rules. 

After this we consider computational aspects of regex and rules with mappings, studying the combined complexity of evaluating extraction expressions over documents. Here we isolate a decision problem which, once solved efficiently, would allow us to enumerate all mappings an expression outputs when matched to a document. Since the size of the answer is potentially exponential here, our objective is to obtain an incremental polynomial time algorithm \cite{johnson1988generating}; an enumeration algorithm that takes polynomial time between each output. As we show, this is generally not possible, but we do isolate a well-behaved fragment, called sequential regex, which properly includes functional regex introduced in \cite{FKRV15}.
We also analyse the evaluation problem parametrized by the number of variables and show that the problem is \emph{fixed parameter tractable}~\cite{FlumG06} for all expressions and automata models we consider.

Finally, we study static analysis of these languages, focusing on satisfiability and containment. While satisfiability is $\NP$-hard for unrestricted languages, the sequentiality restriction introduced when studying evaluation allows us to solve the problem efficiently. On the other hand, containment is bound to be $\PSPACE$-hard, since all of our IE formalisms contain regular expressions, with a matching upper bound giving us completeness for the class. Since one way to lower this bound for regular languages is to consider deterministic models, we show how determinism can be introduced to IE languages and study how it affects the complexity. % of the problem.

%introduce determinism in the context of IE languages, but show that containment can still be difficult in deterministic case. Finally, we identify a semantic restriction which allows us to solve containment efficiently.

\smallskip
\noindent{\bf Organisation.} We define documents, spans and mappings in Section~\ref{sec-prelim}. Expressions and automata for extracting incomplete information are introduced in Section~\ref{sec-unifying}. Expressiveness of our languages is studied in Section~\ref{sec:expr}, and the complexity of their evaluation in Section~\ref{sec:evaluation}. We then tackle static analysis in Section~\ref{sec:complexity} and conclude in Section~\ref{sec-conc}. Due to space limitations most of the proofs are deferred to the appendix.

%\medskip
%\noindent{\bf Organisation.} We define documents, spans and mappings in Section \ref{sec-prelim}. A framework supporting the extraction of incomplete information is introduced in Section \ref{sec-unifying}, where we define different notions of extractions expressions and automata, and show how they are connected. Expressiveness of our languages is studied in Section \ref{sec:expr}, and the complexity of their evaluation in Section \ref{sec:evaluation}. We then tackle static analysis in Section \ref{sec:complexity} and conclude in Section \ref{sec-conc}. Due to space limitations most of the proofs are deferred to the appendix.


==> Rule-Satisfiability.tex <==
\section{Rule satisfiability}

% Rule Satisfiability.
In this section we will describe a procedure for simplifying rules, making them
easier to analyze. This will allow us to derive an algorithm for deciding their
satisfiability.

Throughout most of the section we will only consider \emph{simple} rules and
discuss the \emph{complex} case at the end. We start by showing that
\Treelike{} rules are always satisfiable.
\begin{theorem}
  Let $\theta$ be a rule without body predicates. If $\theta$ is
  \Treelike{} then $\theta$ is satisfiable.
\end{theorem}

\begin{proof}
  We describe an algorithm for constructing a satisfying document $d$ and
  assignment $\sigma$. Set $d \leftarrow \epsilon$ and $\sigma \leftarrow
  \emptyset$. Execute the following procedure, starting with $\varphi_0$, the
  $\SRE$ associated with $\doc$. Given the $\SRE$ $\varphi$ traverse its parse
  tree in pre-order. If the node is a character, append it to $d$. If its a
  disjunction then continue with the left sub-tree only. If its a Kleene star,
  ignore the whole sub-tree. If its a variable $x$, then recursively execute the
  procedure using the $\SRE$ associated with $x$, if it exists, then set
  $\sigma(x)$ to the corresponding span and continue.

  The algorithm is like traversing $G_{\theta}$ in pre-order. Therefore, it will
  always finish since $\theta$ is \Treelike{}. It is also easy to see that
  generated $d$ and $\sigma$ will be satisfying because, given the structure of
  \Treelike{} rules, $\SRE$s will not interfere with each other.
\end{proof}

It would be interesting if we could prove that \Treelike{} rules represent
\emph{exactly} those rules that can be satisfied, that is, that for every
satisfiable rule there is an equivalent \Treelike{} rule. Sadly, that is
not true. To see why, consider the following property of \Treelike{} rules.

\begin{proposition}
  Let \(\theta\) be a simple conjunction and let \(d_1, d_2\) be satisfying
  derivations of \(\theta\). If \(\theta\) is equivalent to a \Treelike{}
  conjunction, then every combination of \(d_1\) and \(d_2\) is satisfying.
\end{proposition}

\begin{proof}
  Let \(\theta'\) be a \Treelike{} conjunction equivalent to \(\theta\).
\end{proof}
\francisco{Finish proof. This sort of has to do with non-trivial dag and
treelike rules being the same.}

Using this fact, we can prove the following two results.

\begin{proposition}
  The \RGX{} formula \(\gamma = ax\{b^{*}\} \vee x\{a^{*}\}b\) cannot be
  expressed using a \Treelike{} rule.
\end{proposition}

\begin{proof}
  Any rule \(\theta\) that tries to express \(\gamma\) must have satisfying
  derivations \(d_1 = \{(\doc, ax), (x, b)\}\) and \(d_2 = \{(\doc, xb), (x,
  a)\}\). Thus, if \(\theta\) is \Treelike{}, \(e = \{(\doc, ax), (x, a)\}\)
  must also be a satisfying derivation for \(\theta\), which means \(\theta\) is
  not equivalent to \(\gamma\).
\end{proof}

\begin{proposition}
  There is a satisfiable rule with that is not equivalent to any \Treelike{}
  rule.
\end{proposition}

\begin{proof}
  Consider the following conjunction:
  \begin{equation*}
    \bm{x}.\bm{y}/\bm{z} \wedge
    \bm{y}.(\bm{w}/\texttt{a}/\bm{z} + \texttt{a}/\bm{z}/\bm{w}) \wedge
    \bm{z}.\epsilon \wedge
    \bm{w}.\Sigma^{*}
  \end{equation*}
  Two satisfying derivations are \(d_1 = \{(x, yz), (y, w\texttt{a}z),
  (z, \epsilon), (w, \texttt{abc})\}\) and \(d_2 = \{(x, yz), (y,\texttt{a}zw),
  (z, \epsilon), (w, \epsilon)\}\). It is easy to see that the combination
  \(e = \{(x, yz), (y, \texttt{a}zw), (z, \epsilon), (w, \texttt{abc})\}\) is
  not satisfying.
\end{proof}

Taking this theorem into account, we will decide the satisfiability of
arbitrary \emph{simple} rules by trying to transform them into \Treelike{}
rules. Given a \emph{simple} rule $\theta$ we will simplify it by inspecting
its graph $G_{\theta}$ and removing undirected cycles from it. We will note
that certain arrangements will only be satisfiable by setting some variables to
$\epsilon$ and thus will allow us to replace some rules and expressions with
simpler ones.

Before proceeding we will emphasize two key properties. Let $\theta$ be a
\emph{simple} rule and $\sigma$ an assignment that satisfies it. We have that,
(1) if $(x,y)$ is an edge in $G_{\theta}$, then $\sigma(y) \sqsubseteq
\sigma(x)$; and (2) if $(x,y)$ and $(x,z)$ are edges in $G_{\theta}$, then
$\sigma(y)$ and $\sigma(z)$ are disjoint. Notice also that two spans are
disjoint and equal if and only if they empty and in the same location.

% Coloring algorithm.

Let $\theta$ be a \emph{simple} rule and let $G_{\theta}$ be its graph. We
define the function $S: \SRE \to \SRE$ as follows.
\begin{align*}
  S(a) &= \emptyset,\quad a \in \Sigma\\
  S(\epsilon) &= \epsilon\\
  S(x) &= x,\quad x \in \Vars\\
  S(\varphi + \psi) &= S(\varphi) + S(\psi)\\
  S(\varphi \cdot \psi) &= S(\varphi) \cdot S(\psi)\\
  S(\varphi^{*}) &= \epsilon
\end{align*}

By further applying the distributive property of concatenation over disjunction
a disjunction of variable strings is obtained. Moreover, if the input $\SRE$ is
\emph{functional}, then every string in the disjunction will contain the same
variables, differing only in their order.

Let $x_i$ and $\varphi_i$ be such that $x_i.\varphi_i$ appears in $\theta$.
Notice that if $S(\varphi_i) = \emptyset$ then $x_i$ for every variable $x_j$
mentioned in $\varphi_i$ and every satisfying valuation $\sigma$ we must have
that $\sigma(x_i)$ strictly contains $\sigma(x_j)$. With this idea in mind, we
will say that a node $x_i$ is \emph{red} if either of the following conditions
is true.
\begin{itemize}
  \item $S(\varphi_i) = \emptyset$.
  \item there exists an edge $(x_i, y)$ such that $y$ is \emph{red}.
\end{itemize}
The node $x_i$ is \emph{green} otherwise. Notice that if a node is \emph{red}
then every satisfying assignment must assign a non-empty span to it.

By analyzing these painted nodes, we may simplify the rule graph. We will
consider directed cycles first. Notice that by the algorithm, this cycles will
be either completely \emph{red} or completely \emph{green}. Let $\theta$ be a
\emph{simple} rule, $\sigma$ an assignment for $\theta$ and $x_1, \ldots, x_n$
the variables that form a directed cycle in $G_{\theta}$. We will denote the
successor of a node $x$ in the cycle as $\Succ(x)$ and we will refer to the
$\SRE$ associated with variable $x$ as $\varphi_x$ (if it exists). Notice the
following properties:
\begin{enumerate}
\item \textbf{The variables in the cycle must be equal.} By transitivity, we
  will have for any two variables $x_i$ and $x_j$ in the cycle that $\sigma(x_i)
  \sqsubseteq \sigma(x_j)$ and $\sigma(x_j) \sqsubseteq \sigma(x_i)$. Therefore
  we must have $\sigma(x_i) = \sigma(x_j)$.

\item \textbf{Every variable reachable from the cycle, but not in it, must
    have empty content.} Let $y$ be a variable reachable from $x_i$. Then, we
  know that $\sigma(y) \sqsubseteq \sigma(x_i)$ and that $\sigma(y)$ is disjoint
  with $\sigma(\Succ(x_i))$. Since $\sigma(x_i) = \sigma(\Succ(x_i))$ the only
  possibility is that $d(\sigma(y)) = \epsilon$.

\item \textbf{If the cycle has a chord, then every variable in it must have
    empty content} Let $x_i$ and $x_j$ be variables from the cycle such that
  $(x_i, x_j)$ is an edge and $\Succ(x_i) \neq x_j$. Then, $\sigma(x_j)$ and
  $\sigma(\Succ(x_i))$ are disjoint, but $\sigma(x_i) = \sigma(\Succ(x_i)) =
  \sigma(x_j)$. Therefore, we must have $\sigma(x_j) = \epsilon$.
\end{enumerate}

Now, we consider the color of cycles.
\begin{itemize}
\item \textbf{If there is a \emph{red} cycle, then the rule is
    unsatisfiable.} If the cycle is \emph{red} then there is a variable $y$ with
  $S(y) = \emptyset$ reachable from some variable $x_i$ in the cycle. This
  implies that $\sigma(\Succ(x_i))$ is strictly contained in $\sigma(x_i)$.
  But $\sigma(x_i) = \sigma(\Succ(x_i))$. Therefore, no such $\sigma$ can exist.

\item \textbf{If there is a \emph{green} cycle, we may simplify it with an
    auxiliary variable.} Let $u_1, \ldots, u_m$ be the variables that are not
  part of the cycle and for which there is an edge $(u_i, x_1)$. Let $y_1,
  \ldots, y_l$ be the variables that are not part of the cycle and are reachable
  from some $x_i$ (they must have empty content, as proved before). We may
  replace the \emph{extraction expressions} for this variables in $\theta$ with
  the following.
  \begin{align*}
    u_i.\varphi_{u_i}[x_1 \rightarrow w], \quad\mbox{ where } 1 \leq i \leq m,\\
    w.x_1,\\
    x_i.S(\varphi_{x_i}), \quad\mbox{ where } 1 \leq i < n,\\
    x_n.S(\varphi_{x_n}[x_1 \rightarrow \Sigma^{*}]),\\
    y_i.\epsilon, \quad\mbox{ where } 1 \leq i \leq l,\\
  \end{align*}
  This yields an equivalent \emph{simple} rule without the mentioned cycle.
\end{itemize}

The last case that we must consider is when we have undirected cycles, that is,
whenever there are two (or more) distinct paths from one node to another. Let
$u$ be the starting node and $v$ the ending node. Let $x_1, \ldots, x_n$ and
$y_1, \ldots, y_m$ be two distinct paths from $u$ to $v$.

Notice, first, that $v$ must have empty content. This is because we have that
$\sigma(x_1)$ and $\sigma(y_1)$ are disjoint, but also $\sigma(v) \sqsubseteq
\sigma(x_1)$ and $\sigma(v) \sqsubseteq \sigma(y_1)$. Therefore, if $\theta$ is
satisfiable, then $d(\sigma(v)) = \epsilon$. In fact, in order for this to be
possible, $v$ must be ``between'' $x_1$ and $y_1$. This observation will allow
us to simplify the rule whenever it's satisfiable.

\begin{itemize}
\item \textbf{If $v$ is \emph{red}, then the rule is unsatisfiable.} As
  proved before, $v$ must have empty content. If $v$ is \emph{red}, then it can
  not have empty content, leading to a contradiction.

\item \textbf{If the rule is satisfiable, then the undirected cycle can be
    eliminated.}

\end{itemize}

==> Spanners.tex <==
%!TEX root = main.tex

\subsection{Comparing expressions to automata}\label{ss-previous}

One of the main problems studied in \cite{FKRV15} was to determine the relationship between the automata models introduced in the previous subsection (restricted to always output relations) with the class of functional \RGX\ formulas. As our framework is an extension (in terms of expressiveness) and a simplification (in terms of semantics) of \cite{FKRV15} that allows mappings instead of simple relations, here we show how the main results on $\fVA$ and $\fRGX$ can be generalised to our setting. %, thus providing us with a sanity check for the extended framework. 
We start by showing that the class of \RGX\ formulas is also captured by $\VAStk$ automata in our new setting.

\begin{theorem}[\cite{FKRV15}]\label{th-stack_rgx}
Every \VAStk\ automaton has an equivalent \RGX\ formula and vice versa. That is $\VAStk \equiv \RGX$.
\end{theorem}

Just as in the proof for the relational case \cite{FKRV15}, the main step is to show that $\VAStk$ automata can be simplified by decomposing them into an (exponential) union of disjoint paths known as $\PUStk$ (path union $\VAStk$). In $\PUStk$ automata each path is essentially a functional \RGX\ formula, thus making the transformation straightforward. The only difference to the proof of \cite{FKRV15} is that when transforming $\VAStk$ automaton into a union of paths, we need to consider all paths of length at most $2\cdot k+1$ in order to accommodate partial mappings, where $k$ is the number of variables. The notion of a consistent path also changes, since we are allowed to open a variable, but never close it. As a corollary we get that every \RGX\ is equivalent to (a potentially exponential) union of functional \RGX\ formulas (with this union being empty when the \RGX\ is not satisfiable).

Similarly as in the functional case, it is also straightforward to prove that the mappings defined by $\VAStk$ and \RGX\ are hierarchical. Furthermore, just as in \cite{FKRV15}, one can show that the class of $\VA$ automata which produce only hierarchical mappings is equivalent to \RGX\ in the general case.

\begin{theorem}[\cite{FKRV15}]\label{th-rgx_equiv_hierarchical_va}
Every \VA\ automaton that is hierarchical has an equivalent \RGX\ formula and vice versa.
\end{theorem}

Both $\VA$ and \VAStk\ automata, as well as \RGX, provide a simple way of extracting information. To permit a more complex way of defining extracted relations, \cite{FKRV15} allows combining them using basic algebraic operations of union, projection and join. While defining a union or projection of two automata or \RGX\ is straightforward, in the case of join we now use joins of mappings instead of the natural join (as used in \cite{FKRV15}). Formally, for two \VA\ automatons $A_1$ and $A_2$, we define the ``join automaton" $A_1\Join A_2$ using the following semantics: for a document $d$, we have $\semd{A_1\Join A_2} = \semd{A_1}\Join \semd{A_2}$. We denote the class of extraction expressions obtained by closing \VA\ under union, projection and join with $\VA^{\{\cup,\pi,\Join\}}$, and similarly for \VAStk\ and \RGX.

To establish a relationship between algebras based on $\VAStk$ and $\VA$ automata, \cite{FKRV15} shows that $\VA$ is closed under union, projection and join. We can show that the same holds true when dealing with mappings, but now the proofs change quite a bit. That is, while closure under  projection is much  easier to prove in our setting, closure under join now requires an exponential blowup, since to join mappings, we need to keep track of variables opened by each mapping in our automaton. Similarly, \cite{FKRV15} shows that each \VA\ automaton can be expressed using the expressions in the algebra $\VAStk^{\{\cup,\pi,\Join\}}$; as this proof holds verbatim in the case of mappings we obtain the following.

\begin{theorem}[\cite{FKRV15}]\label{th-va_algebra_equiv}
$\VA^{\{\cup,\pi,\Join\}}\equiv\VA\equiv\VAStk^{\{\cup,\pi,\Join\}}.$
\end{theorem}

As we showed here, the main results from \cite{FKRV15} can be lifted to hold in the more general setting of mappings, thus suggesting that the added generality does not impact the intuition behind the extraction process. 

%\begin{itemize}
%	\item Hierarchical spanners and operators (Prop 3.14. Page 15).
%	\begin{enumerate}
%		\item The same holds under the new semantics. Not important.
%		\item The same holds under the new semantics. Not important.
%	\end{enumerate}
%	
%	\item Vset and Vset-graphs (Lemma 4.1, Page 16)
%	\begin{enumerate}
%		\item every vstack can be translated into a vstack graph and vice versa. 
%		
%		\item every vset can be translated into a vset graph and vice versa.
%	\end{enumerate}
%	
%	The same holds in our case! Not very important but it is good to mention.
%	
%	\item Vset-graphs and Vset-path union (Lemma 4.2, Page 17)
%	\begin{enumerate}
%		\item every vstack-graph can be translated into a vstack path union and vice versa. 
%		
%		\item every vset-graph can be translated into a vset path union and vice versa.
%	\end{enumerate}
%	Both results holds. The only property that changes is that, instead of considering consistent paths of length $2*k+1$, one has to consider consistent path of length at most $2*k+1$. Here the notion of consistent path also change, because not necessary all variables must be closed.
%	One has to consider here that when the path is constructed, one can remove variables that are open but never closed. 
%	This shows that both semantics are equivalent (that open and closed).
%	
%	\item Vset and Vset-path union (Lemma 4.3, Page 18)
%	This is a corollary of previous results, therefore, also hold verbatim.
%	
%	\item Vstack equivalent to RGX (Theorem 4.4, Page 19) \\
%	The same proof. Here it uses the equivalence with union-vstack-path which also holds for the new semantics.
%	
%	\item hierarchical vset-path are equivalent to vstack-path (Lemma 4.5, page 19, and Theorem 4.6, page 20). \\
%	
%	The reorder of variables can also be done in the new semantics. This is not a property of being functional.
%	
%	\item Union of vset automata (Lemma 4.7, page 20) \\
%	
%	Also straightforward in our case.
%	
%	\item Projection of vset automata (Lemma 4.8, page 20) \\ 
%	
%	The proofs goes by simply ignore with epsilon transition the variable that is projected. In our case the proofs is much simple that the spanner paper, because we don't have the restriction of producing a relation.
%	
%	\item Lexicographic vset-automata (Lemma 4.9, page 22) \\
%	
%	The same proofs holds. The proofs goes by changing the order of variables in path automata. This can also be done with the new semantics.
%	
%	\item * Joins of vset-automata (Lemma 4.10, page 23, Lemma 4.11, page 24) \\
%	
%	We have to be careful here. In the world of mappings, we should consider the join of mappings, which is defined in the paper of Marcelo. Then we can do this operator for mappings but the resulting automata is exponential in the number of variables. This because one has to remember which variables where opened by which mapping. \\ 
%	
%	This result is different.
%	
%	\item Closed under union, projection and natural join. (Theorem 4.12, page 24) \\
%	
%	Stay the same with the new semantics of Join.
%	
%	\item Vset is contained in vstack closed under union, projection and join (Lemma 4.13, page 24). \\
%	
%	The proof is the same. The proof is made on the level of path automata. Since a path automata in our case is ``functional'', then the same construction holds. 
%	
%	\item Equivalence of algebra and vset automata (Theorem 4.14, page 25). \\
%	
%	This is a corollary of previous results, and therefore same proofs holds.
%	
%\end{itemize}

==> Static-Analysis-Complexity.tex <==
% Static analysis and complexity.

\section{Static analysis and complexity}

\subsection{Evaluation}

\Problem
  {\(\nemp(\LL)\)}
  {A document \(d\) and an expression \(\psi \in \LL\).}
  {Is \(\semg{\psi}\) not empty?}

\begin{itemize}
\item \(\nemp(\SRE)\) is \(\NP\)-complete (\cite{AMRV16}).
\item \(\nemp(\SREf)\) is in \(\PTIME\). (Replace variables, run NFA).
\item \(\nemp(\RGX)\) is in \(\PTIME\). (Same).
\item \(\nemp(\text{vset-automata})\) is in \(\NP\). (Checking that run is
  functional is NP-hard? (Hamiltonian path)).
\item \(\nemp(\text{tree-like rule})\) is ?.
\end{itemize}

We also study the complexity of the parameterized versions of these problems.

\begin{itemize}
\item \(\kSRE\) is in \(\FPT\).
\item \(\kRGX\) is in \(\FPT\).
\item \(\nemp(k\text{vset-automata})\) is in \(\FPT\).
\end{itemize}

\subsection{Satisfiability}

\Problem
  {\(\sat(\LL)\)}
  {An expression \(\psi \in \LL\).}
  {Is there a document \(d\) such that \(\semg{\psi}\) is not empty?}

\begin{itemize}
\item \(\sat(\SRE)\) and \(\sat(\text{tree-like})\) are trivial (always
  satisfiable).
\item \(\sat(\RGX)\) is trivial.
\item \(\sat(\text{vset-automata})\) is NP-complete (Hamiltonian path).
\end{itemize}

\subsection{Instance equivalence}

\Problem
  {\(\iequiv(\LL)\)}
  {A document \(d\) and two expressions \(\psi, \gamma \in \LL\).}
  {Is \(\semg{\psi} = \semg{\gamma}\)?}

\begin{itemize}
\item \(\iequiv(\SRE)\) and \(\iequiv(\text{tree-like})\) are in \(\coNP\).
\item \(\iequiv(\RGX)\) is in \(\Pi_2^P\) (any lower?).
\item \(\iequiv(\text{vset-automata})\) is in \(\Pi_2^P\) (any lower?).
\end{itemize}

\subsection{Equivalence}

\Problem
  {\(\eequiv(\LL)\)}
  {Two expressions \(\psi, \gamma \in \LL\).}
  {Is \(\semg{\psi} = \semg{\gamma}\) for every document \(d\)?}

\begin{itemize}
\item \(\eequiv(\SRE)\) is \(\PSPACE\)-hard.
\end{itemize}

==> Variable-Pushdown-Automata.tex <==
% Definition and properties of Variable Pushdown Automata.

\section{Variable Pushdown Automata (\(\VPDA\))}

A Variable Pushdown Automaton (\(\VPDA\)) is a Variable Set Automaton (as
described in~\cite{FKRV15}) augmented with a stack. In this section we propose
three different kinds of \(\VPDA\) with slightly different semantics and
properties.

Formally a \(\VPDA\) is a tuple \((Q, \Sigma, \Gamma, V, \delta, q_0, Z_0, F)\)
where:
\begin{itemize}
  \item \(Q\) is a finite set of \emph{states}.

  \item \(\Sigma\) is a finite set of \emph{input symbols}.

  \item \(\Gamma\) is a finite set of \emph{stack symbols}.

  \item \(V\) is a finite set of \emph{variables}.

  \item \(\delta \subseteq Q \times (\Sigma \cup \{\epsilon\} \cup \{\Open{x},
    \Close{x} \mid x \in V\}) \times \Gamma \times Q \times \Gamma^{*}\) is a
    \emph{transition relation} where tuple \((p, a, X,
    q, \gamma)\) denotes a transition that goes from state \(p\) to state \(q\),
    pops \(X\) from the top of the stack, pushes \(gamma\) to the top of the
    stack, and:
    \begin{itemize}
      \item if \(a \in (\Sigma \cup \{\epsilon\})\), then it reads \(a\) as
        input, or
      \item if \(a = \Open{x}\), then it opens variable \(x\), or
      \item if \(a = \Close{x}\), then it closes variable \(x\).
    \end{itemize}
    
  \item \(q_0 \in Q\) is the \emph{initial state}.

  \item \(Z_0 \in \Gamma\) is the \emph{initial stack symbol}.

  \item \(F \subseteq Q\) is the set of \emph{final states}.
\end{itemize}

A \emph{configuration} of a \(\VPDA\ A\) is a tuple \(c = (q, \alpha, v, y,
i)\), where \(q \in Q\) is the \emph{current state}, \(\alpha \in {(\Gamma \cup
\{\dashv\})}^{*}\) is the \emph{current symbol stack}, \(v \subseteq V\) is the
\emph{active variable set}, \(y \subseteq V\) is the set of \emph{available
variables}, and \(i \in \{1,\ldots,n + 1\}\) is an index indicating the position
of the next character to be read from the input.

A \emph{run} of \(A\) over input \(w = a_1 \ldots a_n\) is a sequence of
configurations \(c_0, \ldots, c_m\) such that \(c_0 = (q_0, Z_0, \epsilon, V,
1)\), and for all \(j \in \{0, \ldots, m - 1\}\) the following holds for
\(c_j = (q_j, \alpha_j, v_j, y_j, i_j)\) and \(c_{j + 1} = (q_{j + 1}, \alpha_{j
+ 1}, v_{j + 1}, y_{j + 1}, i_{j + 1})\):

\begin{itemize}
\item there is a transition \(q_j, b, X, q_{j + 1}, \gamma \in \delta\);
\item \(\alpha_j = X\beta\), and \(\alpha_{j + 1} = \gamma\beta\), for some
  \(\beta \in \Gamma^{*}\);
\item one of the following is true:
  \begin{itemize}
  \item \(v_{j + 1} = v_j\), \(y_{j + 1} = y_j\), \(i_{j + 1} = i_j + 1\), and
    \(b = a_{i_j}\) (ordinary transition), or
  \item \(v_{j + 1} = v_j\), \(y_{j + 1} = y_j\), \(i_{j + 1} = i_j\), and \(b =
    \epsilon\) (epsilon transition), or
  \item \(x \in y_j\), \(v_{j + 1} = v_j \cup \{x\}\), \(y_{j + 1} = y_j
    \setminus \{x\}\), and \(b = \Open{x}\) (variable insert), or
  \item \(x \in y_j\), \(v_{j + 1} = v_j \setminus \{x\}\), \(y_{j + 1} = y_j
    \cup \{x\}\), and \(b = \Close{x}\) (variable remove).
  \end{itemize}
\end{itemize}

A \emph{run} \(\rho = c_0, \ldots, c_m\) is \emph{accepting} if \(c_m = (q,
\alpha, \emptyset, \emptyset, n + 1)\), where \(q \in F\), and \(\alpha \in
\Gamma^{*}\).

\subsection{Context-preserving \(\VPDA\)}

Consider a \emph{run} \(\rho = c_0, \ldots, c_m\) and let \(c_j = (q_j,
\alpha_j, v_j, y_j, i_j)\) for each \(j \in [0, m]\). Given a variable a
variable \(x\) let \(o_x\) be the largest integer such that \(x \in v_{o_x}\)
and let \(c_x\) be the smallest integer such that \(x \in y_{c_x}\). The
\emph{run} \(\rho\) is \emph{context-preserving} if for every variable \(x \in
V\): (1) \(\alpha_{o_x} = \alpha_{c_x}\), and (2) for all \(k \in [o_x, c_x]\)
the stack \(\alpha_{o_x}\) is a suffix of \(\alpha_{k}\).

A \emph{run} is \emph{context-nested} if it is \emph{context-preserving} and
every variable insertion and removal is correctly nested.

\francisco{Define this precisely. Is this condition enough?}

A \emph{context-preserving} \(\VPDA\) (\emph{context-nested} \(\VPDA\)) is a
\(\VPDA\) that only considers \emph{context-preserving runs}
(\emph{context-nested runs}, respectively).


==> intro-old.tex <==
\section{Introduction}
With the abundance of different formats arising in practice these days, there is a great need for methods extracting singular pieces of data from a variety of distinct files. This process, known as information extraction, or IE for short, is particularly prevalent in big corporations that manage systems of increasing complexity which need to incorporate data coming from different sources. As a result, a number of systems supporting the extraction of information from text-like data have appeared throughout the years \cite{KLRRVZ08,Cunningham02,SDNR07}, and the topic received a substantial coverage in the research literature (see \cite{Kimelfeld14} for a good survey).

Historically, there have been two main approaches to information extraction: the {\em statistical} approach utilizing machine-learning methods, and the {\em rule-based} approach utilizing traditional finite-language methods. In this paper we focus on the rule-based approach to information extraction for two reasons. First, rule-based information extraction is founded on methods traditionally used by the database community (such as logic, automata, or datalog-based languages) and has therefore enjoyed a great amount of coverage in the database literature \cite{FKRV15,FKRV14,freydenberger2016document,AMRV16}. Second, as argued by \cite{Kimelfeld14,ChiticariuLR13}, due to their simplicity and ease of use, rule-based systems seem to be more prevalent in the industrial solutions.

Generally, most rule-based information extraction frameworks deploy some form of regular-like expressions as the core mechanism for extracting the data  \cite{CM99,FKRV15,AMRV16}. Perhaps the best representative of this approach are the regular expressions with capture variables introduced in \cite{FKRV15}, called {\em regex formulas}, which form the basis of IBM's commercial IE tool SystemT \cite{KLRRVZ08}. In this setting documents being processed are viewed as strings, which is a natural assumption for a wide variety of formats in use today (e.g. plain text, CSV files, JSON documents, etc.). The pieces of information we want to extract are captured by {\em spans}, which are simply intervals inside the string representing our document (that is, spans are defined by the starting point and the ending point of some substring). Regex formulas are now used to parse these strings, with variables storing {\em spans}.

To make things more concrete, consider a CSV file\footnote{CSV, or comma separated values, is a simple table-like format storing information separated by commas and new lines.} containing land registry records about buyers and sellers. In Table \ref{tab-csv} we give a few rows of such a document, where $\spa$ represents space and $\eol$ the new line symbol.

\begin{table}[h]
\begin{center}
{
\def\arraystretch{1.2}
\renewcommand{\familydefault}{\ttdefault}\normalfont
\begin{tabular}{l}
Seller:$\spa$John,$\spa$ID75\eol\\
{Buyer:}$\spa$Marcelo,$\spa$ID832,$\spa$P78\eol\\
Seller:$\spa$Mark,$\spa$ID7,$\spa$\$35,000\eol\\
\hspace{55pt}$\vdots$
\end{tabular}
}
\end{center}
\vspace*{-15pt}
\caption{Part of a CSV document containing information about buying and selling property.}
\label{tab-csv}
\end{table}

\begin{figure*}[t]
\begin{center}
\resizebox{.85\textwidth}{!}{
\setlength{\tabcolsep}{2pt}
  \renewcommand{\familydefault}{\ttdefault}\normalfont
\begin{tabular}{ccccccccccccccccccccccccccccccccccccccccccccccc}
\small{S} & \small{e} & \small{l} & \small{l} & \small{e} & \small{r} & \small{:} & $\spa$ & \small{J} & \small{o} & \small{h} & \small{n} & \small{,} & $\spa$ & \small{I} & \small{D} & \small{7} & \small{5} & $\eol$ & \small{B} & \small{u} & \small{y} & \small{e} & \small{r} & \small{:} & $\spa$ & \small{M} & \small{a} & \small{r} & \small{c} & \small{e} & \small{l} & \small{o} & \small{,} & $\spa$ & \small{I} & \small{D} & \small{8} & \small{3} & \small{2} & \small{,} & $\spa$ & \small{P} & \small{7} & \small{8} & $\eol$ & $\cdots$\\
\tiny{1} & \tiny{2} & \tiny{3} & \tiny{4} & \tiny{5} & \tiny{6} & \tiny{7} & \tiny{8} &  \tiny{9} & \tiny{10} & \tiny{11} & \tiny{12} & \tiny{13} & \tiny{14} & \tiny{15} & \tiny{16} & \tiny{17} & \tiny{18} & \tiny{19} & \tiny{20} & \tiny{21} & \tiny{22} & \tiny{23} & \tiny{24} & \tiny{25} & \tiny{26} & \tiny{27} & \tiny{28} & \tiny{29} & \tiny{30} & \tiny{31}  & \tiny{32}  & \tiny{33}  & \tiny{34} & \tiny{35} & \tiny{36} & \tiny{37} & \tiny{38} & \tiny{39} & \tiny{40} & \tiny{41} & \tiny{42} & \tiny{43} & \tiny{44} & \tiny{45} & \tiny{46} & 
\end{tabular}
}
\end{center}
\vspace*{-10pt}
\caption{CSV document representing land registry information viewed as a string.}
\label{fig-spandoc}
\end{figure*}

The string representation of this document is given in Figure \ref{fig-spandoc}. 
Suppose that we want to extract the names of sellers from this file. For instance, in the document from Figure \ref{fig-spandoc} we want to capture the span starting at position 9 and ending at position 12 with the content \texttt{John}. This can be accomplished using the regex formula $R_1 := \Sigma^*\cdot\texttt{Seller:}\spa\cdot x\{(\Sigma-\{\texttt{,}\})^*\}\cdot,\cdot\Sigma^*$, which works by locating the position in the document where a seller's name starts (i.e. after the whitespace following the word \texttt{Seller}). It then stores the name into the variable $x$ by stating that the captured span can not contain a comma (as specified by the filter $\{(\Sigma-\{\texttt{,}\})^*\}$). Finally, the expression must now match a comma, and then proceed to the end of the file using $\Sigma^*$.

Once spans have been extracted using regular-like expressions, most IE frameworks allow combining them and controlling their structure through a variety of different methods. For instance, \cite{FKRV15} permits manipulating spans extracted by regex formulas using algebraic operations, while \cite{AMRV16} and \cite{SDNR07} deploy datalog-like programs to obtain a more general way of defining relations over spans. Furthermore, \cite{AMRV16} does not specify the variable filter explicitly inside formulas like regex do, but instead uses a more visual approach implemented through {\em extraction rules}, which permit constraining the shape of a span captured inside a variable $x$ using conjunctions. For instance, if we have an expression $R$ using a variable $x$, extraction rules permit expressions of the form $R\wedge x.R_1 \wedge x.R_2$, stating that the span captured by $x$ also conforms to the expressions $R_1$ and $R_2$.

The way that most frameworks view information extraction is as defining a relation over spans. For example, in regex formulas of \cite{FKRV15} all the variables must be assigned in order to produce an output tuple, and a similar thing happens with the rules-based language of \cite{AMRV16}. However, in practice we are often working with documents which have missing information or optional parts, and would therefore like to maximise the amount of information we wish to extract. Consider for instance the CSV file from Table \ref{tab-csv} containing land registry information. As we can see, some sellers in this file have additional field which contains the amount of tax they paid when selling the property. In an IE setting it might be useful to also obtain this information when it is available. However, if we are set on extracting relations, this will not be possible, since all the variables need to be assigned in order to produce an output.

Apart from the inability to capture partial or incomplete information, some further shortcomings of previous approaches are that defining the semantics of extraction expressions can not be done in a fully declarative way \cite{FKRV15}, or that they assign arbitrary spans to variables when these are not matched against the document \cite{AMRV16}. Furthermore, not much is known how these approaches compare in terms of expressive power, and apart from some preliminary studies on their computational properties \cite{freydenberger2016document,AMRV16}, we do not have a good understanding of how difficult is it to evaluate these languages, nor of the complexity of their main static tasks.

In order to overcome these issues, we propose a general framework subsuming previous approaches to IE, and allowing us to handle incomplete data. We start with regex formulas of \cite{FKRV15} as the base, and redefine their semantics in such a way that they output {\em mappings} in place of relations, much like it was done when defining the semantics of the SPARQL query language in the Semantic Web context \cite{PAG09}. This allows us to capture optional parts of documents, such as in the example above, since our expression will output a mapping that binds an extra variable to the tax data only when the latter is present in the document (otherwise we only extract the name of the seller). Furthermore, the generality of mappings also allows us to have a simple declarative semantics of regex formulas. We also extend the automata models of \cite{FKRV15} to this new setting and show when they capture the extraction expressions we introduce. 

Next, we study how the formal IE frameworks introduced previously compare in terms of expressive power. Here we start with regex formulas of \cite{FKRV15} and span regular expressions of \cite{AMRV16}, since these for the information extraction base of the two frameworks and prove that both are special cases of our definition, with the latter being less expressive. We then analyse extraction rules of \cite{AMRV16} showing how these can be used to capture regex formulas. Note that in our analysis we consider only core extraction mechanisms, such as variants of regular expressions and automata (we plan to examine algebras, and recursive datalog-based languages in the future). Furthermore, we do not consider the content operator of \cite{AMRV16}, nor the string selection of \cite{FKRV15}, since these do not directly extract information, but compare two pieces of existing data.

After this we consider computational aspects of base IE formalisms, starting with evaluation of extraction expressions over documents. Here we isolate a decision problem which, once solved efficiently, would allow us to enumerate all the mappings an expression outputs when matched to a document. Since the size of the answer is potentially exponential here, our objective is to obtain a polynomial delay algorithm \cite{johnson1988generating}. As we show, this is generally not possible, but we do isolate two well-behaved fragments: functional regex formulas of \cite{FKRV15} and sequential tree-like extraction rules of \cite{AMRV16}.

Finally, we study static analysis of these languages, focusing on satisfiability and containment. While satisfiability if $\NP$-hard for general languages, the sequentiality restriction we introduce when studying evaluation allows us to solve the problem efficiently. On the other hand, containment is bound to be $\PSPACE$-hard, since all of our IE formalisms contain regular expressions, with a matching upper bound giving us completeness for the class. Since one way to lower this bound for regular languages is to consider deterministic models, we introduce determinism in the context of IE languages, but show that containment can still be difficult in deterministic case. Finally, we identify a semantic restriction which allows us to solve containment efficiently.


\medskip
\noindent{\bf Organisation.} We define documents, spans and mappings in Section \ref{sec-prelim}. The unifying framework is introduced in Section \ref{sec-unifying}, where we define different notions of extractions expressions and automata and show how are they connected. Expressiveness of IE languages is studied in Section \ref{sec:expr}, and the complexity of their evaluation in Section \ref{sec:evaluation}. We then tackle static analysis in Section \ref{sec:complexity} and conclude in Section \ref{sec-conc}. Due to space limitations most of the proofs are deferred to the appendix.


==> old_eval.tex <==
%!TEX root = main.tex

%\section{Evaluation of IE languages}\label{sec:evaluation}
\section{Evaluation of languages extracting incomplete data}\label{sec:evaluation}


%\cristian{Agregar algoritmo de incremental polynomial time. Discutir la conección con el paper de Freidenberger. Ellos tienen resultados preliminares de complejidad que no se comparan con los nuestros ya que sus resultados no obtienen resultados de incremental polynomial time. Ellos estudian solo model checking lo cual no es suficiente para demostrar incremental polynomial time. }

%\cristian{Agregar la explicación que EVAL incluyen NonEmp y ModelChecking.}

In this section, we study the computational complexity of evaluating an extraction expression $\gamma$ over a document $d$, namely, the complexity of enumerating all mappings $\mu \in \semd{\gamma}$.
Given that we are dealing with an enumeration problem, our objective is to obtain a \emph{polynomial delay} algorithm~\cite{johnson1988generating}, i.e., an algorithm that enumerates all the mappings in $\semd{\gamma}$ by taking  time polynomial in the size of $\gamma$ and $d$ between outputting two consecutive results.
For this analysis, we model our problem as a decision problem and relate it to the enumeration problem.
Formally, let $\bot$ be a new symbol. 
An \emph{extended mapping} $\mu$ over $d$ is a partial function from $\VV$ to $\sub(d) \cup \{\bot\}$.
Intuitively, in our decision problem $\mu(x) = \bot$ will represent that the variable $x$ will not be mapped to any span.
Furthermore, we usually treat $\mu$ as a normal mapping by assuming that $x$ is not in $\dom(\mu)$ for all variables $x$ that are mapped to $\bot$.
Given two extended mappings $\mu$ and $\mu'$, we say that $\mu \subseteq \mu'$ if, and only if, $\mu(x) = \mu'(x)$ for every $x \in \dom(\mu)$. 
%We denote by $\mu_{\downarrow}$ the maximum mapping who satisfies that $\mu_{\downarrow} \subseteq \mu$ and $x \notin \dom(\mu_\downarrow)$ whenever $\mu(x) = \bot$.
Then for any language $\LL$ for information extraction we define the main decision problem for evaluating expressions from $\LL$, called $\EVAL[\LL]$, as follows:
\begin{center}
	\framebox{
		\begin{tabular}{rl}
			\textbf{Problem:} & $\EVAL[\LL]$\\
			\textbf{Input:} &  An expression $\gamma \in \LL$, a document $d$,  \\
			& and an extended mapping $\mu$.  \\
			\textbf{Question:} & Does there exist $\mu'$ such that \\
			&  $\mu \subseteq \mu'$ and  $\mu' \in \semd{\gamma}$?
		\end{tabular}
	}
\end{center}
In other words, in $\EVAL[\LL]$ we want to check whether $\mu$ can be extended to a mapping $\mu'$ that satisfies $\gamma$ in $d$.
Note that in our analysis we will consider the combined complexity of $\EVAL[\LL]$.
%We believe that, although the data complexity of the problem (i.e. the expression $\gamma$ is not part of the input) could derive an interesting insight in the evaluation of extraction expressions, it will not model correctly the complexity in this case.


We claim that $\EVAL[\LL]$ correctly models the problem of enumerating all mappings in $\semd{\gamma}$. 
Indeed, if we can find a polynomial time algorithm for deciding $\EVAL[\LL]$, one can have a polynomial delay algorithm for enumerating the mappings in $\semd{\gamma}$ as given in Algorithm \ref{alg:enum1}.

\begin{algorithm}
  \caption{Enumerate all spans in \(\semd{\gamma}\)}
%  , where \(\mu\) is the current mapping and \(V\) is the set of available variables.}
  \label{alg:enum1}
  \begin{algorithmic}[1]
    \Procedure{Enumerate}{$\gamma, d, \mu, V$}
      \If{\(V = \emptyset\)}
        \State{\textbf{output} \(\mu\) and \Return}
      \EndIf
      \State{Let \(x\) be some element from \(V\)}
      \For{\(s \in \sub(d) \cup \{\bot\}\)}
        \If{\(\EVAL[\LL](\gamma, d, \mu[x \to s])\)}
          \State{
            \Call{Enumerate}{$\gamma, d, \mu[x \to s], V\,\setminus\,\{x\}$}}
        \EndIf
      \EndFor
    \EndProcedure
  \end{algorithmic}
\end{algorithm}

The procedure starts with the empty mapping $\mu = \emptyset$ and the set $V$ of variables yet to be assigned equal to $\Var(\gamma)$. 
For a variable $x \notin \dom(\mu)$ we iterate over all $s \in \sub(d)$ (or the symbol $\bot$ signalling that $x$ is not assigned) and check if $\EVAL[\LL](\gamma, d, \mu[x \rightarrow s])$ is true where $\mu[x \rightarrow s]$ is an extended mapping where $x$ is assigned to $s$ (lines 4 through 6).
If the answer is positive, then in line 7 we recursively continue with the mapping $\mu[x \rightarrow s]$ (i.e. we know that the set of answers is non-empty).
%After iterating over all spans that can be assigned to $x$, the last case is to consider all mappings where $x$ is not assigned (i.e. $x$ is assigned to $\bot$). Thus, we check whether $\EVAL[\LL](\gamma, d, \mu[x \rightarrow \bot])$ holds and continue recursively with $\mu[x \rightarrow \bot]$ if the answer is positive. 
Finally, we print the mapping $\mu$ when all variables in $\Var(\gamma)$ are assigned a span or the symbol $\bot$ (i.e. $V=\emptyset$ in line 2). 
%(i.e. $\dom(\mu) = \Var(\gamma)$). 
%It is straightforward to check that this procedure efficiently enumerates all spans in $\semd{\gamma}$, if we can decide $\EVAL[\LL]$ efficiently. 

We can therefore obtain the following.
\begin{theorem}\label{prop:evaluation}
	If $\EVAL[\LL]$ is in $\PTIME$, then enumerating all mappings in $\semd{\gamma}$ can be done with polynomial delay.
\end{theorem}

Notice that Theorem \ref{prop:evaluation} is a general result allowing us to reason about efficient enumeration of IE languages. That is, when we want to show that {\em any} IE language $\LL$ can be enumerated efficiently, we simply need to show that $\EVAL[\LL]$ is in $\PTIME$. This is in contrast with approaches such as \cite{FKP17}, which, while providing a faster algorithm than the ones we derive below, are applicable to a single fixed language $\LL$. Notice, however, that showing $\EVAL[\LL]$ to be hard does not necessarily rule out the existence of a polynomial delay enumeration procedure for $\LL$.


%On the other hand, if we show that $\EVAL[\LL]$, or any subproblem of $\EVAL[\LL]$, is $\NP$-hard, we automatically get that there is no polynomial delay algorithm for $\LL$ unless $\PTIME=\NP$.

% To show that polynomial delay is not possible we will examine two classical decision problems associated with $\EVAL$; namely, the \emph{model checking problem} and the \emph{non-emptiness problem}.
Two decision problems associated with $\EVAL[\LL]$, that have a long standing history in data management~\cite{AHV95}, are the \emph{model checking problem} and the \emph{non-emptiness problem}. 
Formally, the model checking problem (non-emptiness problem), denoted by $\mdcheck[\LL]$ ($\nemp[\LL]$ resp.), asks whether $\mu \in \semd{\gamma}$ ($\semd{\gamma} \neq \emptyset$ resp.) for any $\gamma \in \LL$, document~$d$ and mapping $\mu$. One can easily see that  both problems are actually restricted instances of $\EVAL[\LL]$, namely:
$$
\renewcommand{\arraystretch}{1.4}
\begin{array}{rcl}
\mdcheck[\LL](\gamma, d, \mu) & = & \EVAL[\LL](\gamma, d, \mu_\bot) \\
\nemp[\LL](\gamma, d) & = & \EVAL[\LL](\gamma, d, \emptyset), 
\end{array}
$$
where $\mu_\bot$ is the extended mapping such that, for all $x \in \Var(\gamma)$, it holds that $\mu_\bot(x) = \mu(x)$ if $x \in \dom(\mu)$ and $\bot$ otherwise.
This implies that if we find an efficient algorithm for $\EVAL[\LL]$ then the same holds for $\mdcheck[\LL]$ and $\nemp[\LL]$. However, solving model checking efficiently does not help us with the enumeration problem and a similar thing holds for non-emptiness.

On the other hand, $\nemp$ can be used as a tool for proving when polynomial delay enumeration is not possible. More precisely, if we can show that $\nemp[\LL]$ is $\NP$-hard, then no polynomial delay algorithm for $\LL$ can exist (under standard complexity assumptions), as we could simply run the enumeration procedure until the first output is produced. 

In contrast, showing $\mdcheck[\LL]$ to be $\NP$-hardness does not necessarily imply that efficient enumeration is not possible, since a polynomial-delay algorithm for enumeration could output the mapping $\mu$ for which we are trying to check whether $\mu \in \semd{\gamma}$ as the final one after exponentially many mappings. As we are interested in efficient enumeration, we will therefore not consider the model checking problem for the remainder of this paper. 

%TALK ABOUT WHAT FREYDENBERGER DID AND HOW WE ADDRESS THIS.
We would like to note that \cite{AMRV16} and \cite{F17} already considered the non-emptiness problem and the model checking problem. In what follows we will point out when a (weaker) version of our results was proved in one of the two works. Generally, we can use \cite{AMRV16,F17} to derive some lower bounds, while we need to show the matching upper bound (when possible) separately. It is important to stress that what \cite{F17} calls evaluation is our model checking problem, and, as discussed above, can not be used to obtain an efficient algorithm for enumeration or $\EVAL$, nor tell us when enumeration with polynomial delay is not possible.

Now that we identified the appropriate decision problems, we start by understanding their complexity in the most general case.
First of all, one can see that checking $\EVAL(\LL)$ is in $\NP$ for all languages and computational models considered in this paper.
Indeed, given a mapping $\mu'$ such that $\mu \subseteq \mu'$ one can check in $\PTIME$ if $\mu' \in \semd{\gamma}$ by using finite automata evaluation techniques~\cite{HopcroftU79}.
As the following result shows, this is the best that one can do if $\RGX$ or variable-set automata contain the language of $\SRGX$, as non emptiness is already hard for this fragment.
\begin{theorem}\label{theo:eval-hardness-general}
$\nemp[\SRGX]$ is $\NP$-comp.
\end{theorem}
We would like to remark that this result was proved in \cite{AMRV16} and here we strengthen it to allow using partial mappings.

%The previous result implies that the evaluation problem for $\RGX$ and variable-set automata is $\NP$-complete. However, it does not say anything about the model checking problem.
%By adapting the proof of the previous result it can be shown that, unfortunately, the model checking problem is also hard for $\RGX$ and variable automata.
%\begin{theorem}\label{theo:model-check}
%  $\mdcheck[\SRGX]$ is $\NP$-complete. %\footnote{This is in contrast with \cite{F17}, where $\mdcheck$ was shown to be in $\PTIME$ for a more general class of expressions.}.
%\end{theorem}


With the previous negative result, we examine several syntactical restrictions of $\RGX$ and variable-set automata that make the evaluation problem tractable.
Note that the previous negative results are considering a more general setting than the one presented in~\cite{FKRV15,F17}, where $\RGX$ and variable-set automata are restricted to be \emph{functional} which forces them to only generate relations of spans. 
Interestingly, the functional restriction decreases the complexity of the non-emptiness and evaluation problem for $\RGX$ as the following result shows.
\begin{proposition}\label{theo:ptime-functional-RGX}
	$\EVAL[\fRGX]$ is in $\PTIME$.
\end{proposition}
This result proves that the functional restriction for $\RGX$ introduced in~\cite{FKRV15} is crucial for getting tractability. 
The question that now remains is what the necessary restrictions are that make the evaluation of $\RGX$ tractable when outputting mappings and how to extend these restrictions to other classes like variable-set automata.
One possible approach is to consider variable-set automata that produce only relations. 
Formally, we say that a variable-set automaton $\cA$ is \emph{relational} if for all documents $d$, the set $\semd{\cA}$ forms a relation. 
As the next result shows, this semantic restriction is not enough to force tractability on $\EVAL[\VA]$.
\begin{proposition}\label{theo:eval-hardness-relational-VA}
	$\nemp$ of relational variable-set automata are $\NP$-complete\footnote{Here $\NP$-hardness of $\nemp$ already follows from the results of \cite{AMRV16,F17}.}.
\end{proposition}
By taking a close look at the proof of the previous result, one can note that a necessary property for getting intractability is that, during a run, the automaton can see the same variable on potential transitions many times but not use it if it has closed the same variable in the past.
Intuitively, this cannot happen in functional $\RGX$ formulas where for every subformula of the form $\varphi_1 \cdot \varphi_2$ it holds that $\Var(\varphi_1) \cap \Var(\varphi_2) =
\emptyset$.
Actually, we claim that this is the restriction that implies tractability for evaluating $\RGX$ formulas. 
Formally, we say that a $\RGX$ formula $\gamma$ is \emph{sequential} if for every subformula of the form $\varphi_1 \cdot \varphi_2$ or $\varphi^*$ it holds that $\Var(\varphi_1) \cap \Var(\varphi_2) =
\emptyset$ and $\Var(\varphi) = \emptyset$, respectively.
We can also extend these ideas of sequentiality from $\RGX$ formulas to variable-set automata as follows.
A path $\pi$ of a variable-set automaton $\cA = (Q, q_0, q_f, \delta)$ is a finite sequence of transitions 
$\pi: (q_1, s_2, q_2), (q_2, s_3, q_3) \ldots, (q_{m-1}, s_m, q_m)$ such that $(q_i, s_{i+1}, q_{i+1}) \in
\delta$ for all $i \in [1, m - 1]$.
We say that a path $\pi$ of $\cA$ is sequential if for every variable \(x \in
\VV\) it holds that: (1) there is at most one \(i \in [1, m]\) such that \(s_i =
\Open{x}\); (2) there is at most one \(j \in [1, m]\) such that \(s_j = \Close{x}\); and (3) if such a \(j\)
exists, then \(i\) exists and \(i < j\).
We say that variable-set automaton $\cA$ is sequential if every path in $\cA$ is sequential.
Finally, we denote the class of sequential RGX and sequential variable-set automata by $\seqRGX$ and $\seqVA$, respectively.

The first natural question about sequentiality is whether this property can be checked efficiently. As the next proposition shows, this is indeed the case.
%sequentiality can be checked in $\NLOGSPACE$.
\begin{proposition}\label{theo:ptime-sequential-check}
	Deciding if a variable-set automaton is sequential can be done in $\NLOGSPACE$.
\end{proposition}

Sequentiality is a mild  restriction over extraction expressions since it still allows many $\RGX$ formulas that are useful in practice.
For example, all extraction expressions discussed in Section~\ref{sec-unifying} are sequential.
Furthermore, as we now show, no expressive power is lost when restricting to sequential \RGX\ or automata. %That is, we can prove the following.
%Furthermore, if we restrict to the fragment of sequential RGX and sequential variable-set automata, we can prove that we will not loose expressive power for extracting information.
\begin{proposition}\label{prop:rgx-equiv-rgx-seq}
For every \RGX\ (\VA\ automaton), there exists a sequential \RGX\ (sequential \VA, respectively) that defines the same extraction function.
\end{proposition}
We believe that sequentiality is a natural syntactical restriction\footnote{Note that \cite{F17} already considers a less general version of sequentiality  called functional VA automata, that open and close all the variables exactly once. There a version of Proposition \ref{theo:ptime-sequential-check} is given with a $\PTIME$ bound, as well as a version of Proposition \ref{prop:rgx-equiv-rgx-seq} for functional automata.} of how to use variables in extraction expressions: in simple terms users should not reuse variables by concatenation since this can easily make the formula unsatisfiable.  Furthermore, the more important advantage for users is that $\RGX$ and variable-set automata that are sequential can be evaluated efficiently. 
\begin{theorem}\label{theo:ptime-sequential-sVA}
	$\EVAL[\seqRGX]$ and $\EVAL[\seqVA]$ is in $\PTIME$.
\end{theorem}
It is important to recall that this result implies, by Theorem~\ref{prop:evaluation}, that enumerating answers of sequential $\RGX$ formulas can be done with polynomial delay. 
Moreover, $\nemp$ of this class can also be decided in $\PTIME$.
This provides us with a good upper-bound for evaluating formulas and shows that it might be possible to find an efficient algorithm that works in practice. With this, we refer to a  \emph{constant delay algorithm}~\cite{johnson1988generating} like the one presented in~\cite{AMRV16} for the so-called navigational formulas -- a class strictly subsumed by sequential $\RGX$.
Thus, sequential $\RGX$ seem like a good direction for extending the constant delay algorithm for navigational formulas given in \cite{AMRV16}.
%
%navigational formulas are a good starting point for the design of constant delay algorithms and sequential $\RGX$ are a good direction for extending them.

Now that we have captured an efficient fragment of \(\RGX\), we will analyse what happens with the complexity of the evaluation problem for extraction rules. First, we show that evaluating rules is in general a hard problem. In fact, non-emptiness is already $\NP$-hard, even when restricted to functional \(\RGX\) and dag-like rules. %, evaluating rules is hard.
\begin{theorem}\label{theo:eval-daglike-npcomplete}
  \(\nemp\) of functional dag-like rules is \(\NP\)-complete.
\end{theorem}
The difficulty in this case arises from the fact that dag-like rules allow referencing the same variable from different extraction expressions. % within the rule. %This makes the evaluation of each extraction expression highly dependent on the other extraction expressions, which makes the problem hard to solve in general.
%
%Therefore, a reasonable restriction in this case is to prohibit variables from being used in multiple extraction expression of the same rule. In other words, we will restrict ourselves to sequential tree-like rules. 
A natural way to circumvent this is to use tree-like rules. 
Indeed, the fact that, in a tree-like rule, different branches are independent, causes the evaluation problem to become tractable.
In fact, the functionality constraint is not really needed here, as the result holds even for sequential rules.
\begin{theorem}\label{theo:treelike-ptime}
  \(\EVAL\) of sequential tree-like rules is in \(\PTIME\).
\end{theorem}

This implies that we should focus on sequential tree-like rules if we wish to have efficient algorithms for rules. Luckily, these do not come at a high price in terms of expressiveness, since Theorem~\ref{thm:simple_to_dag}, Proposition~\ref{prop:nonfunc}, and Theorem~\ref{thm:dag_to_tree} imply that every satisfiable simple rule is equivalent to a union of sequential tree-like rules.

The previous results show how far we can go when syntactically restricting the class of $\RGX$ formulas, variable-set automata, or extraction rules in order to get tractability.
The next step is to parametrize the size of the query not only in terms of the length, but also in terms of meaningful parameters that are usually small in practice. 
In this direction, a natural parameter is the number of variables of a formula or automata since one would expect that this number will not be huge. 
Indeed, if we restrict the number of variables of a $\RGX$ formula or variable-set automata we can show that the problem is fixed parameter tractable.
\begin{theorem}\label{theo:RGX-FPT}
  $\EVAL[\RGX]$ and $\EVAL[\VA]$ para-metrized by the number of variables is $\FPT$.
\end{theorem}
%Similarly, this result can be extended to unrestricted simple extraction rules.
%\begin{theorem}\label{theo:rules-FPT}
%  \(\EVAL\) of extraction rules parame-trized by the number of the number of variables is \(\FPT\).
%\end{theorem}
%The two results show that we can  evaluate all the expressions considered in this paper efficiently when assuming the number of variables to be small.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

